Adaptive Massively Parallel Constant-round Tree Contraction

Miller and Reif's FOCS'85 classic and fundamental tree contraction algorithm is a broadly applicable technique for the parallel solution of a large number of tree problems. Additionally it is also used as an algorithmic design technique for a large number of parallel graph algorithms. In all previously explored models of computation, however, tree contractions have only been achieved in $\Omega(\log n)$ rounds of parallel run time. In this work, we not only introduce a generalized tree contraction method but also show it can be computed highly efficiently in $O(1/\epsilon^3)$ rounds in the Adaptive Massively Parallel Computing (AMPC) setting, where each machine has $O(n^\epsilon)$ local memory for some $0 < \epsilon < 1$. AMPC is a practical extension of Massively Parallel Computing (MPC) which utilizes distributed hash tables. In general, MPC is an abstract model for MapReduce, Hadoop, Spark, and Flume which are currently widely used across industry and has been studied extensively in the theory community in recent years. Last but not least, we show that our results extend to multiple problems on trees, including but not limited to maximum and maximal matching, maximum and maximal independent set, tree isomorphism testing, and more.

==> further-old.tex <==
%\section{Tree Contractions with Bounded Weight}\label{sec:bounded_weight}
\section{Definitions and Terminology}\label{sec:further}

A tree $T=(V,E)$ is given, where $|V| = n$. Assume that $T$ is rooted at vertex $1$, and the vertices are numbered by their index in the preorder traversal of tree $T$, i.e., vertices are numbered $1,2,\ldots, n$ where vertex $i$ is the $i$-th vertex that is visited in the preorder traversal starting from vertex $1$ as root. We can root a tree and also find the preorder numbering of a tree w.h.p. in $O(1/\epsilon)$ AMPC rounds using the techniques mentioned in Behnezhad et. al~\cite{behnezhad2019massively}.

\iffalse
In addition, a weight function $w_T:V \to {\mathbb Z}^{\geq 0}$ is given over the vertices of $T$. 
%Let $t_T$ denote the total weight of the vertices in $V$, i.e., $t_T = \sum_{v\in V}{w_T(v)}$. 
Throughout this paper, we assume the weight function is bounded by the degree of each vertex, i.e., $w_T(v) = O(deg_T(v))$, where $deg_T(v)$ is the degree of vertex $v$ in tree $T$.
Similar to $deg_T$, the weight function $w_T$ is itself a function of $T$, but we show $T$ as a subscript for brevity and we also drop $T$ subscript whenever tree $T$ is implied from the context.

Initially, a binary sequence $D_0^v$ of length $\widetilde{O}(1)$ is stored on each vertex $v \in V$ of a massive tree $T$. The data associated with each vertex $v$ includes the index of $v$ and a reference to its parent. Depending on the problem, $D_0^v$ may contain additional data such as the weight of the edge connecting $v$ to its parent.\footnote{Not to be confused with the weight function $w_T$.} We wish to compute a global property of tree $T$ denoted by $f(D_0^1, D_0^2, \ldots, D_0^n)$, or simply $f(T)$ by exploiting the notation.

Let $\data = \{0, 1\}^*$ be the ground set of possible data values on each vertex. Specifically, say the data at timestep $i$ is a vector $D_i\in \data^{|V_i|}$, where $T_i = (V_i, E_i)$ shows the remaining tree at timestep $i$ as tree $T$ undergoes some modifications during this process. For each timestep $i \geq 1$, $T_i$ must be a minor of $T_{i-1}$, and $T_0 = T$ initially. For some vertex $v\in V_i$, the data at timestep $i$ of $v$ is denoted by $D_i^v \in \data$, which must be a binary sequence of data of length $\widetilde{O}(w_{T_i}(v))$, i.e, $D_i^v \in \{0,1\}^{\widetilde{O}(w_{T_i}(v))}$. 
%Note that $D_i^v$ also contains a reference to $v$ itself. It will additionally start out with a list of the ids of all of $v$'s dependencies (i.e., it's children or descending edges). 
Over the course of the algorithm, $D_i^v$ may be compressed or altered in other ways to satisfy this length constraint.


A \emph{contracting function} $g:2^\data\to \data$ compresses the data associated with a subset of vertices in the tree. 
At a timestep $i \geq 0$ and for a subset $S = \{ v_1,v_2,\ldots,v_k \} \subseteq V_i$, applying $g(D_i^{v_1},\ldots, D_i^{v_k})$ returns a single data entry which is the aggregated data of vertices $v_1, v_2, \ldots, v_k$.
It also modifies the structure of tree $T_i$ so that only one vertex from subset $S$ remains in $T_{i+1}$, which is denoted by $S'$ for any subset $S$. 
Recall that the structure of tree is also stored in $D_i^v$'s by maintaining the parent of each vertex $v$ in $D_i^v$. 
We always assume $S' = v_1$, i.e., the aggregated data of vertices $v_1, v_2, \ldots, v_k$ at timestep $i$ is stored on vertex $v_1$ at timestep $i+1$. 
Hence $D_{i+1}^{v_1} = g(D_i^{v_1},\ldots, D_i^{v_k})$.
We alternatively refer to the set of data stored on vertices in set $S$ by $D_i^S = \{ D_i^{v_1}, D_i^{v_2},\ldots, D_i^{v_k} \}$, and we use the simpler notation $g(D_i^S)$ instead of $g(D_i^{v_1},\ldots, D_i^{v_k})$ when applicable. We define two types of \emph{contracting functions} based on how they modify the structure of tree:
\begin{itemize}
    \item A \emph{``connected contracting function''} is a contracting function which requires the input subset $S = \{ v_1, v_2, \ldots, v_k\}$ induces a connected component, and it contracts the component induced by $S$ into its root (See Definition~\ref{def:connected-contracting}). 
    % After applying a connected contracting function, the connected component induced by $S$ is contracted into $v_1$, where $v_1$ is the root of the induced subtree.
    \item A \emph{``sibling contracting function''} is a contracting function which requires the input subset $S = \{ v_1, v_2, \ldots, v_k\}$ be a \emph{leaf-star}, a collection of leaves sharing the same parent. Applying a \emph{sibling contracting function} on a leaf-star removes all but one of leaves. We will later discuss why defining this type of contracting functions is necessary and formally define it in Definition~\ref{def:sibling-contracting}.
\end{itemize}
\fi

%Applying $g(D_i^{v_1},\ldots, D_i^{v_k})$ at some $i$ for some $S = \{ v_1,v_2,\ldots,v_k \} \subseteq V_i$, contracts vertices in $S$ into a single vertex in $T_{i+1}$ which we call $S'$. We also always assume $S' = v_1$, i.e., vertices $v_2, \ldots, v_k$ are contracted into vertex $v_1$.
%Let $v_1$ be the root of the subtree induced by $S$. 
%Then, $g(D_i^{v_1},\ldots, D_i^{v_k})$ returns the data of $v_1$ at timestep $i+1$, $D_{i+1}^{v_1}$, which is the compression of $(D_i^{v_1},\ldots, D_i^{v_k})$ based off contracting $v_1,\ldots,v_k$. 

% We require that $S$ is connected. 
%We alternatively refer to the contracted vertex $v_1$ which represents component $S$ in $T_{i+1}$ by $S'$.

%$S = V\times R$ where $r\in R$ is a valid data you could have for one vertex. $f: 2^S\to S$
%%$(v_1, D(v_1))\times(v_2,D(v_2))\times\ldots()\into()$
%on tree $T$ works only on a connected subgraph $S \subseteq T$, and evaluates a partial solution for $S$ which will be stored in vertex $S'$ in $T'$, where $T'$ is created by contracting subgraph $S$ into a single vertex $S'$.

\subsection{Contracting Functions}\label{sec:contracting-functions}

In Section~\ref{sec:preliminaries}, we defined \emph{contracting functions} (Definition~\ref{def:contracting-function}) and briefly mentioned two types of contracting functions, namely \emph{connected contracting functions} and \emph{sibling contracting functions}. In this section, we formally define the two types of contracting functions and discuss why the existence of sibling contracting functions is necessary in some cases. 
% Moreover, we formally define \emph{valid collections of contracting functions} (Definition~\ref{def:valid}) and \emph{$w$-bounded collection of contracting functions} (Definition~\ref{def:w-bounded}).


\begin{definition}\label{def:connected-contracting}
A \emph{``connected contracting function''} $g:2^\data\to\data$ is a contracting function which requires that the input $(D_i^{v_1}, D_i^{v_2}, \ldots,D_i^{v_k})$ at timestep $i$ corresponds to a subset $S = \{ v_1, v_2, \ldots, v_k \} \subseteq V_i$ which induces a connected component rooted at $v_1$ in $T_i$. Applying $g(D_i^S)$, contracts the subtree induced by $S$ into $v_1$ such that $D_{i+1}^{v_1} = g(D_i^S)$.
\end{definition}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[c]{0.55\textwidth}
        \centering
        \includegraphics[scale=0.025]{images/treeC.png}
        \caption{Tree $T_i$, and subset $S$ are illustrated in this figure. Each red vertex is a member of $S$.}
        \label{fig:treeC}
    \end{subfigure}\qquad
    \begin{subfigure}[c]{0.35\textwidth}
        \centering
        \includegraphics[scale=0.025]{images/treeCX.png}
        \caption{This figure illustrates tree $T_{i+1}$ which is created by contracting the component induced by $S$. The contracted vertex $S' = 1$ is colored red, and we have $D_{i+1}^{S'} = g(D_i^S)$.}
        \label{fig:treeCX}
    \end{subfigure}
    \caption{An example tree $T_i$ is illustrated in (\ref{fig:treeC}). The red vertices show the subset $S$ which induces a connected component. Applying a \emph{connected contracting function} $g$ contracts the component induced by $S$ in into its root $S' = 1$. Tree $T_{i+1}$ and the contracted vertex $S'$ are illustrated in (\ref{fig:treeCX}).} 
    \label{fig:contracting}
\end{figure}

Note that a \emph{connected contracting function} might have additional requirements for the input subset. For example, assume we are given two connected contracting functions $\C$ and $\R$ for \blackbox{Compress} and \blackbox{Rake} stages of Tree Contraction respectively. Although $\C$ potentially admits any subset $S$ as long as it induces a connected components in the tree, $\R$ requires that the input subset $S$ induces a star. We sometimes call functions like $\R$ a connected contracting Rake function to emphasize this distinction.

%A connected contracting function $g$ is a \emph{valid contracting function} with respect to any function $f$ if repeated applications of $g$ on connected components of $T$ in any order until it is contracted into a single vertex results in $f(T)$. In other words, $f(D_i) = f(D_{i+1})$ for any timestep $i$ assuming the only difference between $D_i$ and $D_{i+1}$ is an application of $g$ at timestep $i$ on subset $S = \{ v_1, v_2, \ldots, v_k \}$. We define valid contracting functions formally in Definition~\ref{def:valid}.
%if for any tree $T$ and any $i$ repeated applications of $f$ on components of $T$ in any order until it is contracted into a single point results in data that contains a solution to $\mathcal{P}$ on $T$.  

%A \emph{valid contracting function} $f$ returns the correct output when $T$ is contracted into a single vertex using possibly several application of function $f$ on connected subgraphs, no matter which subgraphs or in which order we contract. \hamed{More details about \emph{valid contracting functions} from memory and output point of view}

We would like to remark that in some cases having efficient connected contracting functions $\R$ and $\C$ is not sufficient for designing an efficient tree contraction algorithm for a given function $f$ in the AMPC model. 
Ideally, we need to contract a huge number of connected components simultaneously at each timestep $i$ to utilize the parallelization power of the AMPC model.
However, the chosen components at any timestep $i$ must be disjoint. Otherwise, several different components might end up contracting into the same vertex. As an example, consider the entire input tree $T$ is a star with $n-1$ leaves centered at vertex $1$. In this example, any non-trivial connected component, containing at least two nodes, includes vertex $1$. Hence, at least $O(n^{1-\epsilon})$ timesteps are required to contract $T$ into a single vertex if we are able to contract at most $O(n^\epsilon)$ leaves at a time.

To overcome this obstacle, we define a slightly different kind of contracting functions called \emph{sibling contracting functions}. Recall that a \emph{``leaf-star''} is a set of at least $2$ leaves sharing a common parent. A \emph{sibling contracting function} $g: 2^\data \to \data$ compresses the data associated with the leaves in a leaf-star. Consider a leaf-star $S = \{ v_1, v_2, \ldots, v_k \}$. By definition, $|D_i^{v_j}| = \widetilde{O}(1)$ for all $j \in [k]$ since all $v_j$'s are leaves. $g(D_i^{v_1},D_i^{v_2},\ldots,D_i^{v_k})$ returns the aggregated data of $v_1,v_2,\ldots,v_k$, which again by definition must have length at most $\widetilde{O}(1)$, based off removing all the leaves in this leaf-star except $v_1$. Assume the aggregated data is stored in $D_{i+1}^{v_1}$ in timestep $i+1$. Note that the subgraph induced by $S$ is not connected, and a sibling contracting function does not technically contracts the subgraph induced on $S$. 
% We also define \emph{valid leaf-star shrinking functions} similar to \emph{valid contracting functions}, and say a \emph{valid leaf-star shrinking function} $\R$ is ``$w$-bounded'' if for any timestep $i$ and any leaf-star made of leaves $v_1,v_2,\ldots,v_k$ in $T_i$, the following holds:
% \[|D_{i+1}^{v_1}| = |\R(D_i^{v_1},D_i^{v_2},\ldots,D_i^{v_k})| = \widetilde{O}\left(w_{T_{i+1}}(v_1)\right) = \widetilde{O}(1)\]
% Likewise, we assume $|D_{i}^{v_j}| = \widetilde{O}\left(w_{T_i}(v_j)\right) = \widetilde{O}(1)$ for any $j \in [k]$.

\begin{definition}\label{def:sibling-contracting}
A \emph{``sibling contracting function''} $g:2^\data\to\data$ is a contracting function which requires that the the input $(D_i^{v_1}, D_i^{v_2}, \ldots,D_i^{v_k})$ at timestep $i$ corresponds to a subset $S = \{ v_1, v_2, \ldots, v_k \} \subseteq V_i$ which is a \emph{leaf-star}. Applying $g(D_i^S)$, aggregates the data of $v_1, v_2, \ldots, v_k$ into $v_1$, i.e., $D_{i+1}^{v_1} = g(D_i^S)$, and removes vertices $v_2, v_3, \ldots, v_k$ from $T_i$ to obtain $T_{i+1}$.

 A subset $S = \{ v_1, v_2, \ldots, v_k \} \subseteq V_i$ is a \emph{``leaf-star''} if $v_i$ is a leaf for all $i \in [k]$, and all $v_i$'s have the same parent $u \in V_i$.
%A \emph{``connected contracting function''} $g:2^\data\to\data$ is a contracting function which requires that the input $(D_i^{v_1}, D_i^{v_2}, \ldots,D_i^{v_k})$ at timestep $i$ corresponds to a subset $S = \{ v_1, v_2, \ldots, v_k \} \subseteq V_i$ which induces a connected component rooted at $v_1$ in $T_i$. Applying $g(D_i^S)$, contracts the subtree induced by $S$ into $v_1$ such that $D_{i+1}^{v_1} = g(D_i^S)$.
\end{definition}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[c]{0.50\textwidth}
        \centering
        \includegraphics[scale=0.025]{images/treeR.png}
        \caption{Tree $T_i$, and subsets $S_1$, $S_2$, and $S_3$ are illustrated in this figure. Each blue vertex belongs to a $S_j$ for some $j \in \{ 1,2,3 \}$.}
        \label{fig:treeR}
    \end{subfigure}\qquad
    \begin{subfigure}[c]{0.40\textwidth}
        \centering
        \includegraphics[scale=0.025]{images/treeRX.png}
        \caption{This figure illustrates tree $T_{i+1}$ which is created by aggregating the leaf-stars $S_1$, $S_2$, and $S_3$. The contracted vertices $S'_1$, $S'_2$, and $S'_3$ are colored blue, and we have $D_{i+1}^{S_j'} = g(D_i^{S_j})$ for any $j \in \{1,2,3\}$.}
        \label{fig:treeRX}
    \end{subfigure}
    \caption{The same tree $T_i$ from Figure~\ref{fig:contracting} is illustrated in (\ref{fig:treeR}). The blue vertices show three \emph{leaf-stars} $S_1$, $S_2$, and $S_3$. Applying a \emph{sibling contracting function} $g$ on $S_1$, $S_2$, and $S_3$ respectively aggregates the leaves in each leaf-star into  $S'_1$, $S'_2$, and $S'_3$. Tree $T_{i+1}$ and the contracted vertices $S'_1$, $S'_2$, and $S'_3$ are illustrated in (\ref{fig:treeCX}).} 
    \label{fig:leafstar}
\end{figure}

\subsection{Preorder Decomposition}\label{subsec:decompose}

To start, we wish to find a decomposition of vertices $V_1, V_2, \ldots, V_k \subseteq V$ of a given tree $T=(V,E)$ ($\cup_{i=1}^k{V_i} = V$ and $V_i \cap V_j = \phi \;\;\forall{i,j}: i \neq j$) so that for all ${i \in [n]}$, $w(V_i) = O(\lambda)$ for a given parameter $\lambda$. Assume the weight function $w$ is \emph{weight-bounded}, i.e., $w(v) = O(\lambda)$ for all $v \in V$. For the simplicity of notation $w$ is also defined on subsets as $w(S) = \sum_{v\in S}{w(v)} \;\; \forall{S \subseteq V}$. Roughly speaking, our approach is to apply Compress function $\C$ on each connected component of every group $V_i$ to reduce the number of vertices. In this section, we show that using a special decomposition of vertices, called  \emph{preorder decomposition}, for which $w(V_i) = O(\lambda)$ for all $i \in [k]$ leads to an efficient AMPC algorithm for computing any arbitrary function $f(T)$ which satisfy a specific set of constraints.

Assume that the vertices are numbered by their index in the preorder traversal of tree $T$, i.e., vertices are numbered $1,2,\ldots, n$ where vertex $i$ is the $i$-th vertex that is visited in the preorder traversal starting from vertex $1$ as root. We can find the preorder numbering of a tree w.h.p. in $O(1/\epsilon)$ AMPC rounds using the techniques mentioned in Behnezhad et. al~\cite{behnezhad2019massively}. In a \emph{preorder decomposition} of $T$, each group $V_i$ consists of a consecutive set of vertices in the preorder numbering of the vertices. More precisely, let $l_i$ denote the index of the vertex $v \in V_i$ with the largest index, and assume $l_0 = 0$ for consistency. In a preorder decomposition, group $V_i$ consists of vertices $l_{i-1} + 1, l_{i-1} + 2, \ldots, l_{i}$. Recall that the vertices are numbered from $1$ to $n$ based on the order they appear in the \emph{preorder traversal} of $T$ starting from vertex $1$ as root.

\begin{definition}\label{def:preorder-dependency}
Given a tree $T=(V,E)$, a \emph{``preorder decomposition''} $V_1,V_2,\ldots,V_k$ of $T$ is defined by a vector $l \in \mathbb{Z}^{k+1}$, such that $0 = l_0 < l_1 < \ldots < l_k = n$, as $V_i = \{l_{i-1}+1,l_{i-1}+2,\ldots,l_i\}\;\; \forall{i \in [k]}$. See Subfigure~\ref{fig:preorder} for an example.
\end{definition}

\begin{observation}\label{obs:groups}
In any given tree $T = (V, E)$ along with any weight function $w:V \to \mathbb{Z}^{\geq 0}$ and a parameter $\lambda$ such that $w(v) = O(\lambda)$ for all $v \in V$, there is a preorder decomposition $V_1, V_2, \ldots, V_k$ so that $w(V_i) = O(\lambda) \;\;\forall{i \in [k]}$ and $k = O(n/\lambda)$.
%\marina{shouldnt we just require $w(v)>0$ and simplify this to $k\leq O(t/s)$? also i think this argument is easier of we say $w(V_i) \leq 2s$, which is okay to do. it just needs to be $O(s)$ really} \hamed{I think we require $w(v) < s$ in this part right? Also the reason I used $\max(n,t)$ was that for some weight function $t$  can be smaller than $n$. However, we could assume $t$ is always $O(n)$ and use $n$ instead of $\max(n,t)$. About the other part, yeah that is also possible but I wasn't planning to show any proof here.}\marina{oh I wasn't saying we shouldn't say $w(v) < s$, i jsut think if we add the constraint $w(v)>0$ instead of $w(v)\geq 0$, because then $t$ cannot be smaller than $n$. when would we ever need ti to be smaller than $n$? } \hamed{Oh, I see. Yeah we probably never want to have $t < n$, but in section 3 when we set $w(v)$ to be the number of children each vertex, $w(v) = 0$ for each leaf $v$. But yeah it would be nice if we simplify $O(\max(n,t)/s)$ somehow.}
\end{observation}

For example, let $w(v) = 1$ for every vertex. Then each group $V_i$ of a preorder decomposition contains at most $O(\lambda)$ vertices, and there exists a preorder decomposition with at most $O(n/\lambda)$ groups. Another example is to define $w(v)$ to be the number of the children of each vertex in tree $T$. Here, the number of edges $e = (p, v)$ such that the parent $p$ is included in group $V_i$ is bounded by $O(\lambda)$ as long as there is no vertex with $\omega(\lambda)$ children in $T$. 
It is easy to observe that no matter how $w(v)$ is defined, as long as $w(v) = O(\min(\lambda,\degr(v)))$ for all $v \in V$, we can greedily group vertices into a \emph{preorder decomposition} $V_1, V_2, \ldots, V_k$ as desired in Observation~\ref{obs:groups}.
% In this paper, we almost always assume $t = \tilde{O}(n)$. Simplify: we have $w(v) \leq d(v)$!

The dependency tree $T'=(V', E')$ of a decomposition $V_1, V_2, \ldots, V_k$ is defined over the connected components within the induced subgraph of each group as vertices. For each $i \in [k]$, let $F_i$ show the forest that is induced by $V_i$. There exists one vertex in $V'$ for each connected component $C_{i,1}, \ldots, C_{i,c_i}$ in every $F_i$, where $c_i$ denotes the number of connected components in $F_i$. Define $T'$ to be the tree that is constructed by contracting every connected component $C_{i,j}$ for all $i \in [k], j \in [c_i]$. 
%Note that this is in fact a tree, as components $C_{i,j}$ cannot be a descendant of $C_{i',j'}$ for $i'>i$, thus $T'$ contains no cycles. \hamed{Dependency tree is not necessarily defined for a \emph{preorder} decomposition, so this argument is invalid. However, we always get a tree if we contract some connected subgraphs of a tree.} 
We call a component $C_{i,j}$ \emph{independent} if the node $C'_{i,j}$ representing this component in $T'$ is a leaf, and otherwise we call it a \emph{dependent} component. Again, for any connected subgraph $S \subseteq T$ we contract, we denote the corresponding contracted node in $T'$ by $S'$.

\begin{definition}\label{def:dependency-tree}
Given a tree $T=(V, E)$ and a decomposition of vertices $V_1,V_2,\ldots,V_k$, the \emph{``dependency tree''} $T'=(V',E')$ of $T$ under this decomposition is constructed by contracting each connected component $C_{i,j}$ for all $j \in [c_i]$ in each group $V_i$. We call a component contracted to a leaf in $T'$ an \emph{``independent''} component, and a component contracted to a non-leaf vertex in $T'$ a \emph{``dependent''} component.
\end{definition}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.50\textwidth}
        \centering
        \includegraphics[scale=0.055]{preorder-decomposition.png}
        \caption{A preorder decomposition of $T$ into $V_1,V_2,\ldots,V_7$ with $w(v)=1$ and $\lambda = 4$. Edges within any $F_i$ are depicted bold, and edges belonging to no $F_i$ are depicted dashed.}
        \label{fig:preorder}
    \end{subfigure}\qquad
    \begin{subfigure}[b]{0.40\textwidth}
        \centering
        \includegraphics[scale=0.065]{dependency-tree.png}
        \caption{Dependency tree $T'$, created by contracting connected components of every $F_i$. Each red vertex represents a dependent component, and each white vertex represents an independent component.}
        \label{fig:dependency}
    \end{subfigure}
    \caption{In Subfigure (\subref{fig:preorder}), a preorder decomposition of a given tree $T$ is demonstrated. Based on this preorder decomposition, we define a dependency tree $T'$ so that each connected component $S$ in each forest $F_i$ is contracted into a single vertex $S'$. This dependency tree $T'$ is demonstrated in Subfigure (\subref{fig:dependency}). It is easy to observe that the contracted components are maximal components which are connected using bold edges in $T$, and each edge in $T'$ corresponds to a dashed edge in $T$.} 
    \label{fig:my_label}
\end{figure}

\begin{lemma}\label{lemma:preorder-decomposition}
The dependency tree $T'=(V',E')$ of a preorder decomposition $V_1, V_2, \ldots, V_k$ of tree $T=(V,E)$ contains at most $1$ non-leaf vertex per group for a total of at most $k$ non-leaf vertices. In other words, there are at most $k$ dependent connected components in $\cup_{i\in[k]}{F_i}$.
\end{lemma}
\begin{proof}
Each group $V_i$ induces a forest $F_i$ on tree $T$, and recall that each $F_i$ is consisted of multiple connected components $C_{i,1}, C_{i,2}, \ldots, C_{i, c_i}$, where $c_i$ is the number of connected components of $F_i$. Assume w.l.o.g. component $C_{i,c_i}$ is the component which contains vertex $l_i$, the vertex with the largest index in $V_i$. We show that every connected component in $F_i$ except $C_{i,c_i}$ is independent, and thus Lemma~\ref{lemma:preorder-decomposition} statement is implied. See in Subfigure~\ref{fig:dependency} that there is at most $1$ dependent component, red vertices in $T'$, for each group $V_i$. Also note that $C_{i,c_i}$, the only possibly dependent component in $F_i$, is always the last component if we sort the components based on their starting index since $l_i \in C_{i,c_i}$ and each $C_{i,j}$ contains a consecutive set of vertices.

Assume for contradiction that there exists $C_{i,j}$ for some $i \in [k], j \in [c_i-1]$, a non-last component in group $V_i$, such that $C_{i,j}$ is a dependent component, or equivalently $C'_{i,j}$ is not a leaf in $T'$. 
Since $C_{i,j}$ is a dependent component, there is a vertex $v \in C_{i,j}$ which has a child outside of $V_i$. Let $u$ be the first such child of $v$ in the pre-order traversal, and thus $u \in V_j$ for some $j > i$. Consider a vertex $w \in V_i$ that comes after $v$ in the pre-order traversal.
Then, since $u$, and thus $V_j$, comes after $v$ and $V_i$ in the pre-order traversal, $u$ must come after $w$ in the pre-order traversal. Since $w$ is between $v$ and $u$ in the pre-order traversal, and $u$ is a child of $v$, the only option is for $w$ to be a descendant of $v$. Then the path from $w$ to $v$ consists of $w$, $w$'s parent $p(w)$, $p(w)$'s parent, and so on until we reach $v$. Since a parent always comes before a child in a pre-order traversal, all the intermediate vertices on the path from $w$ to $v$ come between $w$ and $v$ in the pre-order traversal, so they must all be in $V_i$. This means $w$ is in $C_{i,j}$ since $w$ is connected to $v$ in $F_i$. Since any vertex after $v$ in $V_i$ must be in $C_{i,j}$, $C_{i,j}$ must be the last connected component, i.e., $j=c_i$. This implies that the only possibly dependent connected component of $F_i$ is $C_{i,c_i}$, and all other $C_{i,j}$'s for $j \in [c_i-1]$ are independent.
\end{proof}


==> further.tex <==

\newpage
%\section{Tree Contractions with Bounded Weight}\label{sec:bounded_weight}
\section{Definitions and Terminology}\label{sec:further}




\subsection{Preorder Decomposition}\label{subsec:decompose}

To start, we wish to find a decomposition of vertices $V_1, V_2, \ldots, V_k \subseteq V$ of a given tree $T=(V,E)$ ($\cup_{i=1}^k{V_i} = V$ and $V_i \cap V_j = \phi \;\;\forall{i,j}: i \neq j$) so that for all ${i \in [n]}$, $w(V_i) = O(\lambda)$ for a given parameter $\lambda$. Assume the weight function $w$ is \emph{weight-bounded}, i.e., $w(v) = O(\lambda)$ for all $v \in V$. For the simplicity of notation $w$ is also defined on subsets as $w(S) = \sum_{v\in S}{w(v)} \;\; \forall{S \subseteq V}$. Roughly speaking, our approach is to apply Compress function $\C$ on each connected component of every group $V_i$ to reduce the number of vertices. In this section, we show that using a special decomposition of vertices, called  \emph{preorder decomposition}, for which $w(V_i) = O(\lambda)$ for all $i \in [k]$ leads to an efficient AMPC algorithm for computing any arbitrary function $f(T)$ which satisfy a specific set of constraints.

Assume that the vertices are numbered by their index in the preorder traversal of tree $T$, i.e., vertices are numbered $1,2,\ldots, n$ where vertex $i$ is the $i$-th vertex that is visited in the preorder traversal starting from vertex $1$ as root. We can find the preorder numbering of a tree w.h.p. in $O(1/\epsilon)$ AMPC rounds using the techniques mentioned in Behnezhad et. al~\cite{behnezhad2019massively}. In a \emph{preorder decomposition} of $T$, each group $V_i$ consists of a consecutive set of vertices in the preorder numbering of the vertices. More precisely, let $l_i$ denote the index of the vertex $v \in V_i$ with the largest index, and assume $l_0 = 0$ for consistency. In a preorder decomposition, group $V_i$ consists of vertices $l_{i-1} + 1, l_{i-1} + 2, \ldots, l_{i}$. Recall that the vertices are numbered from $1$ to $n$ based on the order they appear in the \emph{preorder traversal} of $T$ starting from vertex $1$ as root.

\begin{definition}\label{def:preorder-dependency}
Given a tree $T=(V,E)$, a \emph{``preorder decomposition''} $V_1,V_2,\ldots,V_k$ of $T$ is defined by a vector $l \in \mathbb{Z}^{k+1}$, such that $0 = l_0 < l_1 < \ldots < l_k = n$, as $V_i = \{l_{i-1}+1,l_{i-1}+2,\ldots,l_i\}\;\; \forall{i \in [k]}$. See Subfigure~\ref{fig:preorder} for an example.
\end{definition}

\begin{observation}\label{obs:groups}
In any given tree $T = (V, E)$ along with any weight function $w:V \to \mathbb{Z}^{\geq 0}$ and a parameter $\lambda$ such that $w(v) = O(\lambda)$ for all $v \in V$, there is a preorder decomposition $V_1, V_2, \ldots, V_k$ so that $w(V_i) = O(\lambda) \;\;\forall{i \in [k]}$ and $k = O(n/\lambda)$.
%\marina{shouldnt we just require $w(v)>0$ and simplify this to $k\leq O(t/s)$? also i think this argument is easier of we say $w(V_i) \leq 2s$, which is okay to do. it just needs to be $O(s)$ really} \hamed{I think we require $w(v) < s$ in this part right? Also the reason I used $\max(n,t)$ was that for some weight function $t$  can be smaller than $n$. However, we could assume $t$ is always $O(n)$ and use $n$ instead of $\max(n,t)$. About the other part, yeah that is also possible but I wasn't planning to show any proof here.}\marina{oh I wasn't saying we shouldn't say $w(v) < s$, i jsut think if we add the constraint $w(v)>0$ instead of $w(v)\geq 0$, because then $t$ cannot be smaller than $n$. when would we ever need ti to be smaller than $n$? } \hamed{Oh, I see. Yeah we probably never want to have $t < n$, but in section 3 when we set $w(v)$ to be the number of children each vertex, $w(v) = 0$ for each leaf $v$. But yeah it would be nice if we simplify $O(\max(n,t)/s)$ somehow.}
\end{observation}

For example, let $w(v) = 1$ for every vertex. Then each group $V_i$ of a preorder decomposition contains at most $O(\lambda)$ vertices, and there exists a preorder decomposition with at most $O(n/\lambda)$ groups. Another example is to define $w(v)$ to be the number of the children of each vertex in tree $T$. Here, the number of edges $e = (p, v)$ such that the parent $p$ is included in group $V_i$ is bounded by $O(\lambda)$ as long as there is no vertex with $\omega(\lambda)$ children in $T$. 
It is easy to observe that no matter how $w(v)$ is defined, as long as $w(v) = O(\min(\lambda,\degr(v)))$ for all $v \in V$, we can greedily group vertices into a \emph{preorder decomposition} $V_1, V_2, \ldots, V_k$ as desired in Observation~\ref{obs:groups}.
% In this paper, we almost always assume $t = \tilde{O}(n)$. Simplify: we have $w(v) \leq d(v)$!

The dependency tree $T'=(V', E')$ of a decomposition $V_1, V_2, \ldots, V_k$ is defined over the connected components within the induced subgraph of each group as vertices. For each $i \in [k]$, let $F_i$ show the forest that is induced by $V_i$. There exists one vertex in $V'$ for each connected component $C_{i,1}, \ldots, C_{i,c_i}$ in every $F_i$, where $c_i$ denotes the number of connected components in $F_i$. Define $T'$ to be the tree that is constructed by contracting every connected component $C_{i,j}$ for all $i \in [k], j \in [c_i]$. 
%Note that this is in fact a tree, as components $C_{i,j}$ cannot be a descendant of $C_{i',j'}$ for $i'>i$, thus $T'$ contains no cycles. \hamed{Dependency tree is not necessarily defined for a \emph{preorder} decomposition, so this argument is invalid. However, we always get a tree if we contract some connected subgraphs of a tree.} 
We call a component $C_{i,j}$ \emph{independent} if the node $C'_{i,j}$ representing this component in $T'$ is a leaf, and otherwise we call it a \emph{dependent} component. Again, for any connected subgraph $S \subseteq T$ we contract, we denote the corresponding contracted node in $T'$ by $S'$.

\begin{definition}\label{def:dependency-tree}
Given a tree $T=(V, E)$ and a decomposition of vertices $V_1,V_2,\ldots,V_k$, the \emph{``dependency tree''} $T'=(V',E')$ of $T$ under this decomposition is constructed by contracting each connected component $C_{i,j}$ for all $j \in [c_i]$ in each group $V_i$. We call a component contracted to a leaf in $T'$ an \emph{``independent''} component, and a component contracted to a non-leaf vertex in $T'$ a \emph{``dependent''} component.
\end{definition}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.50\textwidth}
        \centering
        \includegraphics[scale=0.055]{preorder-decomposition.png}
        \caption{A preorder decomposition of $T$ into $V_1,V_2,\ldots,V_7$ with $w(v)=1$ and $\lambda = 4$. Edges within any $F_i$ are depicted bold, and edges belonging to no $F_i$ are depicted dashed.}
        \label{fig:preorder}
    \end{subfigure}\qquad
    \begin{subfigure}[b]{0.40\textwidth}
        \centering
        \includegraphics[scale=0.065]{dependency-tree.png}
        \caption{Dependency tree $T'$, created by contracting connected components of every $F_i$. Each red vertex represents a dependent component, and each white vertex represents an independent component.}
        \label{fig:dependency}
    \end{subfigure}
    \caption{In Subfigure (\subref{fig:preorder}), a preorder decomposition of a given tree $T$ is demonstrated. Based on this preorder decomposition, we define a dependency tree $T'$ so that each connected component $S$ in each forest $F_i$ is contracted into a single vertex $S'$. This dependency tree $T'$ is demonstrated in Subfigure (\subref{fig:dependency}). It is easy to observe that the contracted components are maximal components which are connected using bold edges in $T$, and each edge in $T'$ corresponds to a dashed edge in $T$.} 
    \label{fig:my_label}
\end{figure}

\begin{lemma}\label{lemma:preorder-decomposition}
The dependency tree $T'=(V',E')$ of a preorder decomposition $V_1, V_2, \ldots, V_k$ of tree $T=(V,E)$ contains at most $1$ non-leaf vertex per group for a total of at most $k$ non-leaf vertices. In other words, there are at most $k$ dependent connected components in $\cup_{i\in[k]}{F_i}$.
\end{lemma}
\begin{proof}
Each group $V_i$ induces a forest $F_i$ on tree $T$, and recall that each $F_i$ is consisted of multiple connected components $C_{i,1}, C_{i,2}, \ldots, C_{i, c_i}$, where $c_i$ is the number of connected components of $F_i$. Assume w.l.o.g. component $C_{i,c_i}$ is the component which contains vertex $l_i$, the vertex with the largest index in $V_i$. We show that every connected component in $F_i$ except $C_{i,c_i}$ is independent, and thus Lemma~\ref{lemma:preorder-decomposition} statement is implied. See in Subfigure~\ref{fig:dependency} that there is at most $1$ dependent component, red vertices in $T'$, for each group $V_i$. Also note that $C_{i,c_i}$, the only possibly dependent component in $F_i$, is always the last component if we sort the components based on their starting index since $l_i \in C_{i,c_i}$ and each $C_{i,j}$ contains a consecutive set of vertices.

Assume for contradiction that there exists $C_{i,j}$ for some $i \in [k], j \in [c_i-1]$, a non-last component in group $V_i$, such that $C_{i,j}$ is a dependent component, or equivalently $C'_{i,j}$ is not a leaf in $T'$. 
Since $C_{i,j}$ is a dependent component, there is a vertex $v \in C_{i,j}$ which has a child outside of $V_i$. Let $u$ be the first such child of $v$ in the pre-order traversal, and thus $u \in V_j$ for some $j > i$. Consider a vertex $w \in V_i$ that comes after $v$ in the pre-order traversal.
Then, since $u$, and thus $V_j$, comes after $v$ and $V_i$ in the pre-order traversal, $u$ must come after $w$ in the pre-order traversal. Since $w$ is between $v$ and $u$ in the pre-order traversal, and $u$ is a child of $v$, the only option is for $w$ to be a descendant of $v$. Then the path from $w$ to $v$ consists of $w$, $w$'s parent $p(w)$, $p(w)$'s parent, and so on until we reach $v$. Since a parent always comes before a child in a pre-order traversal, all the intermediate vertices on the path from $w$ to $v$ come between $w$ and $v$ in the pre-order traversal, so they must all be in $V_i$. This means $w$ is in $C_{i,j}$ since $w$ is connected to $v$ in $F_i$. Since any vertex after $v$ in $V_i$ must be in $C_{i,j}$, $C_{i,j}$ must be the last connected component, i.e., $j=c_i$. This implies that the only possibly dependent connected component of $F_i$ is $C_{i,c_i}$, and all other $C_{i,j}$'s for $j \in [c_i-1]$ are independent.
\end{proof}


==> preliminaries-old.tex <==
\section{Preliminaries}\label{sec:preliminaries}
\iffalse
A rooted tree $T=(V,E)$ is given, where $|V| = n$, and let $p_T(v)$ and $\children_T(v)$ show the parent of $v$ and the set of the children of $v$ for each vertex $v \in V$. Throughout this paper, the degree of a vertex $v$, denoted by $\degr_T(v)$, is defined as the number of its children and it does not include its parent, i.e., $\degr_T(v) = |\children_T(v)|$. We omit the $T$ subscript whenever tree $T$ is implied from the context.
The goal is to compute a global property of $T$, say $f(T)$, in a very few parallel rounds. Our approach is to extend the \emph{Tree Contraction} framework to run in a constant number of rounds in the AMPC model.

\emph{Tree Contraction} is originally introduced by Miller and Reif~\cite{miller1989parallel}. 
At a high level, their framework provides the means to compute a global property with respect to a given tree in $O(\log{n})$ \emph{phases}.
In each \emph{phase}, there are two \emph{stages}:

\begin{itemize}
    \item \compress{} stage: Contract around half of the vertices with degree $1$ into their parent.
    \item \rake{} stage: Contract all the leaves (vertices with degree $0$) into their parent.
\end{itemize}

Repeated applications of \compress{} and \rake{} alternatively results in a tree which has only one vertex. 
Intuitively, the \compress{} stage aims at shortening the long \emph{chains}, maximal connected sequences of vertices whose degree is equal to $1$, and the \rake{} stages cleans up the leaves.
Both stages are necessary in order to guarantee that $O(\log{n})$ phases are enough to end up with a single remaining vertex~\cite{miller1989parallel}. 

In the original variant, every odd-indexed vertex of each \emph{chain}
is contracted in a \compress{} stage. In some randomized variants, each vertex is selected with probability $1/2$ independently, and an independent set of the selected vertices is contracted. In such variants, contracting two consecutive vertices in a chain is avoided in order to efficiently implement the tree contraction in the PRAM model. However, this restriction is not imposed in the AMPC model, and hence we consider a more \emph{relaxed variant} of the \compress{} stage where each maximal chain is contracted into a single vertex.

\subsection{Generalized Tree Contraction}

We introduce a more generalized version of tree contraction as follows: In \emph{$\alpha$-tree-contraction}, the \rake{} stage is the same as before, but in the \compress{} stage, every maximal subgraph containing only vertices with degree less than $\alpha$ is contracted into a single vertex.

\begin{definition}\label{def:alpha-tc}
In an $\alpha$-tree-contraction of a tree $T=(V,E)$, we repeat two stages in a number of phases until the whole tree is contracted into a single vertex:
\begin{itemize}
    \item \blackbox{Compress} stage: Contract every maximal connected component $S$ containing only vertices with degree less than $\alpha$, i.e., $\degr(v)<\alpha\;\;\forall{v \in S}$, into a single vertex $S'$.
    \item \blackbox{Rake} stage: Contract all the leaves into their parent.
\end{itemize}
\end{definition}

Notice that the relaxed variant of Miller and Reif's \compress{} stage is the special case when $\alpha=2$. Our goal will be to implement efficient $\alpha$-tree-contraction where $\alpha=n^\epsilon$, as this will give us the desired complexity. 
Interestingly, it is possible to solve a broad range of DP formulation on trees in $O(1/\epsilon^2)$ AMPC rounds using $n^\epsilon$-tree-contraction. 
% \hamed{Ref to max matching as an example} 
Similar to the fact that the number of tree contraction phases is bounded by $O(\log(n))$ in $2$-tree-contraction, we show an upper bound of $O(1/\epsilon)$ for the number of phases in $n^\epsilon$-tree-contraction. More generally, we provide an upper bound for $\alpha$-tree-contraction in Lemma~\ref{lemma:rounds}. The proof of Lemma~\ref{lemma:rounds} is deferred to appendix~\ref{sec:main}.

\begin{restatable}{lemma}{alpharounds}\label{lemma:rounds}
For any $\alpha \geq 2$, the number of $\alpha$-tree-contraction phases until we have a constant number of vertices is bounded by $O(\log_{\alpha}(n))$.
\end{restatable}
\fi


While \compress{} and \rake{} (Defined in Section~\ref{subsec:tree-contraction}) describe the process of contracting the tree structure, in order to solve actual problems on trees, we require intermediate functions for \compress{} and \rake{} operations that maintain compressed partial solutions as we contract the tree. We call such intermediate functions \emph{contracting functions}.
But before defining contracting functions formally, we need to specify how \textit{data} is stored at each vertex of the tree. 
Initially, a binary sequence $D_0^v$ of length $\widetilde{O}(\degr_T(v))$ is stored on each vertex $v \in V$ of a tree $T$. Recall that $\degr_T(v)$ is the degree of vertex $v$. The data associated with each vertex $v$ includes the index of $v$ and a collection of references to its parent and its children. Depending on the problem, $D_0^v$ may contain additional data such as the weight of the edge connecting $v$ to its parent. %\footnote{Not to be confused with the weight function $w_T$ we will define shortly.}
At the end of this process, we retrieve $f(D_0^1, D_0^2, \ldots, D_0^n)$ (or simply $f(T)$ by exploiting the notation), a global property of tree $T$, from the aggregated \textit{data} stored in the root of the tree.

However, for a global property $f(T)$ to admit an \textit{efficient} tree contraction algorithm, the \emph{contracting functions} for \compress{} and \rake{} must be space efficient.
To address this, we limit the size of \emph{data} we are allowed to store at each vertex $v$ by the current degree of $v$ throughout the algorithm.  
%To address this, we define a weight function $w_T:V \to {\mathbb Z}^{\geq 0}$ over the vertices of $T$ with respect to the global property we wish to compute.  
%In a sense, our weight function $w_T$ limits the size of \emph{data} we are allowed to store at each vertex of $T$.
%Throughout this paper, we assume the weight function is bounded by the degree of each vertex, i.e., $w_T(v) = O(\degr_T(v))$.
%Similar to $\degr_T$, the weight function $w_T$ is itself a function of $T$, but we show $T$ as a subscript for brevity and we also drop $T$ subscript whenever tree $T$ is implied from the context.
Let $\data = \{0, 1\}^*$ be the ground set of possible data values on each vertex. Specifically, say the data at timestep $i$ is a vector $D_i\in \data^{|V_i|}$ and $T_i = (V_i, E_i)$ is the remaining tree at timestep $i$. To start, $T_0=T$. For each timestep $i \geq 1$, $T_i$ must be a minor\footnote{Graph $H$ is a minor of graph $G$ if it can be formed by starting progressively deleting edges and vertices and contracting edges. In this work, we only use contractions. Note that a minor of a tree is a tree.} of $T_{i-1}$. For some vertex $v\in V_i$, the data at timestep $i$ of $v$ is denoted by $D_i^v \in \data$, which must be a binary sequence of length $\widetilde{O}(\degr_{T_i}(v))$, i.e, $D_i^v \in \{0,1\}^{\widetilde{O}(\degr_{T_i}(v))}$. 
%Note that $D_i^v$ also contains a reference to $v$ itself. It will additionally start out with a list of the ids of all of $v$'s dependencies (i.e., it's children or descending edges). 
Over the course of the algorithm, $D_i^v$ may be compressed or altered in other ways to satisfy this length constraint.
Now we are ready to define \emph{contracting functions} formally.

\begin{definition}\label{def:contracting-function}
A \emph{``contracting function''} $g:2^\data\to \data$ compresses the data associated with a subset of vertices in the tree. 
At a timestep $i \geq 0$ and for a subset $S = \{ v_1,v_2,\ldots,v_k \} \subseteq V_i$, applying $g(D_i^{v_1},\ldots, D_i^{v_k})$ returns a single data entry which is the aggregated data of vertices $v_1, v_2, \ldots, v_k$.
It also modifies the structure of tree $T_i$ so that only one vertex from subset $S$ remains in $T_{i+1}$, which is denoted by $S'$ for any subset $S$. 
\end{definition}

Recall that the structure of tree is also stored in the $D_i^v$s by maintaining the neighbors of each vertex $v$ in $D_i^v$. 
We always assume $S' = v_1$, i.e., the aggregated data of vertices $v_1, v_2, \ldots, v_k$ at timestep $i$ is stored on vertex $v_1$ at timestep $i+1$. 
Hence $D_{i+1}^{v_1} = g(D_i^{v_1},\ldots, D_i^{v_k})$.
We alternatively refer to the set of data stored on vertices in set $S$ by $D_i^S = \{ D_i^{v_1}, D_i^{v_2},\ldots, D_i^{v_k} \}$, and we use the simpler notation $g(D_i^S)$ instead of $g(D_i^{v_1},\ldots, D_i^{v_k})$ when applicable. We define two types of \emph{contracting functions} based on how they modify the structure of tree:
\begin{itemize}
   \item A \emph{``connected contracting function''} is a contracting function which requires that the input subset $S = \{ v_1, v_2, \ldots, v_k\}$ induces a connected component and it contracts the component induced by $S$ into its root. 
    After applying a connected contracting function, the connected component induced by $S$ is contracted into $v_1$, where $v_1$ is the root of the induced subtree. See Definition~\ref{def:connected-contracting} for a formal definition.
    \item A \emph{``sibling contracting function''} is a contracting function which requires the input subset $S = \{ v_1, v_2, \ldots, v_k\}$ be a \emph{leaf-star},
    a collection of leaves sharing the same parent not including the parent itself. Applying a \emph{sibling contracting function} on a leaf-star removes all but one of leaves. We will later discuss why defining this type of contracting functions is necessary and will formally define it in Definition~\ref{def:sibling-contracting}.
\end{itemize}

\iffalse
It turns out that given a connected contracting function and a sibling contracting function, it is much simpler to contract a internal component of the tree in the \compress{} phase--simply apply the connected contracting function and contract the component into a single vertex. \rake{}, on the other hand, requires more care and may utilize both functions. This breaks down into two specific cases. For each leaf-star, \rake{} must efficiently compress all the leaf-children of a leaf-star parent into the parent itself. This can be problematic if the leaves in a leaf-star cannot fit onto one machine. For our first, simpler case, we consider when all leaf-stars only enough children to fit on one machine. This is proposed in Algorithm~\ref{alg:connected-rake}.\footnote{See Section~\ref{subsec:w-bounded} for additional notation.}

Algorithm~\ref{alg:connected-rake} is sufficient to implement \rake{} on trees with bounded degree with specified properties. However, we will also need to implement \rake{} on high-degree trees where the data can be efficiently compressed into size $O(1)$. In order to handle vertices with more than $O(n^\epsilon)$, we could theoretically apply Algorithm~\ref{alg:connected-rake} $O(1/\epsilon)$ times. However, in order to avoid this round-complexity blowup, we can leverage the sibling contracting function to avoid sequential applications of a contracting function. This is depicted in Algorithm~\ref{alg:sibling-rake}.\footnote{See Section~\ref{subsec:w-bounded} for additional notation.}

Together, these functions allow us to implement both \compress{} and \rake{}. In order to solve dynamic programming on trees, one must propose problem-specific connected and sibling contracting functions. We will later prove that such functions can be designed for a number of algorithms.
\fi

See Appendix~\ref{sec:further} for a formal definition of the aforementioned types of contracting functions.

\subsection{\Degres{}  property}\label{subsec:w-bounded}

A connected contracting function $g$ is a \emph{valid contracting function} with respect to an arbitrary function $f$ if repeated applications of $g$ on connected components of $T$ in any order until it is contracted into a single vertex results in $f(T)$. In other words, $f(D_i) = f(D_{i+1})$ for any timestep $i$ assuming the only difference between $D_i$ and $D_{i+1}$ is an application of $g$ at timestep $i$ on subset $S = \{ v_1, v_2, \ldots, v_k \}$. 
%We define valid contracting functions formally in Definition~\ref{def:valid}.
%if for any tree $T$ and any $i$ repeated applications of $f$ on components of $T$ in any order until it is contracted into a single point results in data that contains a solution to $\mathcal{P}$ on $T$.

We extend the definition \emph{valid contracting functions} to a collection of contracting functions, possibly including \emph{sibling contracting functions}. Note that we need to have at least one connected contracting function, otherwise we can't collapse $T$ into a single vertex. In this paper, we often use at least, but not limited to, two contracting function at the same time to contract a tree. As an example we may have a Compress function $\C$ and Rake function $\R$ which both are \emph{connected contracting functions}. We need to ensure that applying both functions in any order on a given tree still results in $f(T)$ when the tree collapses into a single vertex. In some other cases, the Rake function $\R$ is given as a \emph{sibling contracting function}, yet we need to make sure it works correctly in conjunction with given $\C$.

\begin{definition}\label{def:valid}
A collection of contracting functions $\mathcal{G} = \{ g_1, g_2, \ldots, g_l \}$ is a \emph{``valid'' collection of contracting functions} with respect to a given function $f$ we wish to compute if there exists a sequence of applications of $g_j$'s such that $T$ is collapsed into a single vertex, and any such sequence results in $f(T)$. In other words, $f(D_i) = f(D_{i+1})$ for any timestep $i$ assuming the only difference between $D_i$ and $D_{i+1}$ is an application of a $g_j \in \mathcal{G}$ at timestep $i$ on a subset $S = \{ v_1, v_2, \ldots, v_k \}$ which $g_j$ admits, i.e., $V_{i+1} = V_i \setminus \{ v_2, v_3, \ldots, v_k \}$, $D_{i+1}^{v_1} = g_j(D_i^{v_1},\ldots, D_i^{v_k})$, $D_{i+1}^{v} = D_{i}^v$ for all $v \in V_{i+1} \setminus \{ v_1 \}$, and $T_i$ is modified into $T_{i+1}$ depending on the type of $g_j$. 
\end{definition}

In order to efficiently utilize a \emph{valid collection of  contracting functions} $\mathcal{G} = \{ g_1, g_2, \ldots, g_l \}$ in the AMPC model, we need to impose some memory restrictions on each $g_i$, which we briefly mentioned before. In a nutshell, we restrict each contracting function to output a data entry with size proportional to the degree of the contracted vertex in the next timestep. More concretely, we require $D_i^v$ to be a binary sequence of length $\widetilde{O}(\degr_{T_i}(v))$ for any vertex $v \in V_i$ at any timestep $i \geq 0$, and we wish any sequence of applications of contracting functions in $\mathcal{G}$ maintains this condition given that it is satisfied for its input vertices. In Definition~\ref{def:w-bounded}, we define the \emph{\degres{}} property for a valid collection of contracting functions to address this restriction.


\begin{definition}\label{def:w-bounded}
A \emph{valid collection of contracting functions} $\mathcal{G} = \{ g_1, g_2, \ldots, g_l \}$ is \emph{``\degres''} if \[|D_{i+1}^{v_1}| = |g_j(D_i^S)| = \widetilde{O}\left(\degr_{T_{i+1}}(v_1)\right)\] 
for any $g_j \in \mathcal{G}$ on any subsets $S =  \{ v_1, \ldots, v_k \}$ in $T_i$ which $g_j$ admits at timestep $i$, given that $|D_i^{v_j}| = \widetilde{O}\left(\degr_{T_i}(v_j)\right)$ for any $j \in [k]$.
\end{definition}

Note that in Definition~\ref{def:w-bounded}, the  bound on the memory complexity of the data associated with $v_1$ after applying $g_j(D_i^S)$ depends on the degree of vertex $v_1$ in tree $T_{i+1}$ of the next timestep $i+1$, i.e.,  $\degr_{T_{i+1}}(v_1)$. For instance, if 
%$w$ is defined to be the number of children of each vertex and 
$T_i$ is a binary tree, then contracting an arbitrary connected component $S$ can increase $\degr_{T_{i+1}}(S')$ to way more than $2$, while $\degr_{T_i}(v) \leq 2\;\;\forall{v\in S}$. 
Another extreme example is when $T_i$ is a star rooted at center, 
%, the weight function $w$ is the same, 
and $S$ is the whole graph except one leaf. In the latter example, the available memory to store $D_{i+1}^{S'}$ decreases from $\widetilde{O}(\degr_{T_i}(S)) = \widetilde{O}(n)$ to $\widetilde{O}(\degr_{T_{i+1}}(S')) = \widetilde{O}(1)$ after contracting the subtree induced by $S$ into a single vertex $S'$. This example further motivates the definition of \emph{sibling contracting functions} which aggregate the data stored in a subset of leaves, potentially in parallel, without touching the data in the parent vertex.



\iffalse
Let the vertex set at phase $i$ be $V_i$, with $V_0=V$. Then the \emph{data} stored at vertex $v$ in phase $i$, denoted $D_i^v$, is some binary sequence stored on the vertex itself in the tree. Let $\mathcal{D}$ be the set of possible data values on any vertex. Then the vector of all data on our tree at phase $i$ is $D_i\in \mathcal{D}^{|V_i|}$. This data $D_i^v$ is intended to represent the solution to the subtree rooted at $v$. To illustrate this process using a simple running example problem, consider the problem where every leaf $\ell \in \leaves(V_0)$ ($\leaves(S)$ denotes the set of leaves in a subgraph induced by a vertex set $S$), is assigned an arbitrary value $\val(\ell)$, and the value of an internal node is recursively defined as the sum of the values of its children:
\begin{align*}
\forall v\in V \setminus \leaves(V_0):&\,\, \val(v) = \sum_{u\in \children(v)} \val(u),
\end{align*}

The goal is to compute the value of the root. We refer to this problem as \textsf{SumParent}, whose input and output is depicted in Figures~\ref{fig:sumparenta} and~\ref{fig:sumparentb}. Then for all leaves $\ell\in \leaves(V_0)$, let $D_0^\ell = \val(\ell)$. For any internal node $v$, we will simply let $D_0^v$ be a small tree with root $v$ and leaves $\children(v)$, coupled with a number. If $T_v$ is that tree, then $D_0^v= (T_v, \val(v))$, where $\val(v)$ starts out as 0. Over the course of the algorithm, $\val(v)$ will increase until it reaches the true value of vertex $v$. Notice that in this example, $|D_0^v| = O(\degr_T(v))$, so the data for $v$ can be stored in $\widetilde{O}(\degr_T(v))$ bits. The data of our example tree can be seen in the first row of Figure~\ref{fig:sumparentc}.

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[scale=0.035]{images/sumparent1.png}
        \caption{An example input tree to \sumparent. The leaves are initialized with values, and all vertices are labeled with an index.}
        \label{fig:sumparenta}
    \end{subfigure}\qquad
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[scale=0.035]{images/sumparent2.png}
        \caption{The solution to the \sumparent example. Each vertex is labeled with its final value. We are interested in the root value.}
        \label{fig:sumparentb}
    \end{subfigure}\qquad
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[scale=0.035]{images/sumparent4.png}
        \caption{To solve the tree, we apply \compress{} and \rake{}. This is what the tree looks like after compressing vertices $2$ and $3$ and then raking vertices $8$ and $9$.}
        \label{fig:sumparentd}
    \end{subfigure}\\
        \begin{subfigure}[c]{0.9\textwidth}
        \centering
        \includegraphics[scale=0.05]{images/sumparent3.png}
        \caption{This table depicts the data stored at each value at the start of the algorithm (row 1), after compressing vertices $2$ and $3$ (row 2), and after raking vertices $8$ and $9$ (row 3).}
        \label{fig:sumparentc}
    \end{subfigure}
        \caption{Running example for \textsf{Sumparent}. We illustrate simply compressing the component consisting of vertices $2$ and $3$ and then raking leaves $8$ and $9$.} 
    \label{fig:sumparent}
\end{figure}
Next, we consider how the data transforms throughout the \compress{} and \rake{} process. We start by describing the \compress{} stage. Recall that \compress{} compresses all components of low degree simultaneously, but let us just consider compressing a component that consists of just vertices $2$ and $3$ from Figure~\ref{fig:sumparenta}. Notice that since $\val(2)$ is a sum that involves $\val(3)$ and $\val(3)$ is just the sum of the values of its children, $\val(2)$ depends on the children of vertex $3$ in the same way $\val(3)$ does. So without changing the numeric data at vertex $2$, we can simply compress vertex $3$ into vertex $2$, and allow vertex $2$ to take on vertex $3$'s children. This change is depicted in the second row of Figure~\ref{fig:sumparentc}. 

Now we describe how \rake{} executes. As in our description for \compress{}, we note that \rake{} removes all leaves simultaneously, however we will just consider the leaves incident to vertex $1$. There are two such leaves: $8$ and $9$. Since $\val(1)$ is a sum involving $\val(8)$ and $\val(9)$, and we have immediate access to $\val(8)$ and $\val(9)$ (this must be true because they are leaves), we can modify the data of vertex $1$ as follows: remove vertices $8$ and $9$ from the tree, and add $\val(8)$ and $\val(9)$ to the running value at vertex $1$. This change is depicted in the third row of Figure~\ref{fig:sumparentc}, and the resulting tree after the described partial \compress{} and \rake{} is shown in Figure~\ref{fig:sumparentd}. We could continue doing \compress{} and \rake{} stages in this manner until we contract all components into the root, and then the final \rake{} will give us the value at the root.

Ultimately, \textsf{SumParent} is solvable using tree contractions because we can formulate what we call a \textit{contracting function}. In what follows, we informally define \emph{contracting functions} and some related notions. See appendix~\ref{sec:preliminaries} for formal definitions. A contracting function $g:2^\mathcal{D}\to \mathcal{D}$ takes multiple data values of a component of a subtree and compresses them into a single data value representing the compression of the component. In the case of \compress{}, we contract an entire internal component of a subtree into its root, and in the case of \rake{}, we contract leaves into a parent. For example, in \textsf{SumParent}, our data at a vertex $v$ looks like $D_i^v=(T_v, \val(v))$, as we store both a small tree (which may be empty, and otherwise is a star) and a running value. The contracting function for \compress{} of a component $S$ with root $r$ is $\C(D_i^S) = (T_r', \val(r) + \sum_{\ell\in \leaves(S)} \val(\ell))$, where $T_r'$ is a star graph with root $r$ and leaves that are $\children(S)\setminus S$. By exploiting the notation, $\children(S)$ is defined for a subtree $S$ as $\cup_{v\in S}{\children{v}}$. The contracting function for \rake{} of a parent $v$ and its leaf children $u_1,\ldots,u_k$ would look like $\R(D_i^v,D_i^{u_1},\ldots,D_i^{u_k}) = (T_v',\val(v) + \sum_{i\in [k]} \val(u_k))$, where $T_v'$ trims off its leaves $u_1,\ldots,u_k$. 

A \emph{connected contracting function} $g$ is a \emph{``valid contracting function''} with respect to a global property $f(T)$ if repeated applications of $g$ on connected components of $T$ in any order until it is contracted into a single vertex results in $f(T)$. In other words, $f(D_i) = f(D_{i+1})$ for any timestep $i$ assuming the only difference between $D_i$ and $D_{i+1}$ is an application of $g$ at timestep $i$ on subset $S = \{ v_1, v_2, \ldots, v_k \}$. Note that a \emph{sibling contracting function} by itself cannot be a valid contracting function since repeated applications of a sibling contracting function will not reduce a tree $T$ into a single vertex. Hence, we extend our definition of validity to a collection of contracting functions.

A \emph{collection of contracting functions}, say $\mathcal{G}=\{\C, \R\}$, may include a connected contracting function $\C$, for using in the \compress{} stage, as well as a sibling contracting function $\R$, for using in the \rake{} stage.
We say a collection of contracting functions $\mathcal{G}=\{\C, \R\}$ is a \textit{``valid collection of contracting functions''} with respect to a global property $f(T)$ to be one such that if we repeatedly apply $\C$ and $\R$ to subgraphs of $T_i$s in any order until we reach a single vertex, we always end up with $f(T)$. \footnote{Note that if we want to solve some problems, like we will show for maximum matching and others, we may use tree contractions to find a value \textit{other} than the solution to the problem. This value should then be able to be used to efficiently solve the given problem.}  For a formal definition of a valid collection of contracting functions see Definition~\ref{def:valid} in Appendix~\ref{sec:further}.
%It is not hard to see that the set of proposed contracting functions for \textsf{SumParent} is indeed valid. Then, if we iteratively execute \compress{} and \rake{} using $\C$ and $\R$ to modify tree data along the way, we will eventually end up with a single vertex, the root $v_0$, with data $(\{v_0\}, \val(v_0))$, and thus we have solved \textsf{SumParent}.

% However, for a contraction function to yield an \textit{efficient} tree contraction algorithm, the contracting functions for \compress{} and \rake{} must be space efficient. To address this, we introduce the notion of a \textit{$w$-bounded} collection of contracting functions.

%In a sense, our weight function $w$ defines the size of the compressed data of a contracted component. Ultimately, this will help us argue that our algorithms can be distributed onto machines with sublinear memory constraints. Now we have enough foundations to discuss our results.

In order to efficiently utilize a \emph{valid collection of  contracting functions} $\mathcal{G} = \{ \C, \R \}$ in the AMPC model, we need to impose some memory restrictions on each $g_i$, which we briefly mentioned before. In a nutshell, we restrict each contracting function to output a data entry with size proportional to the weight of the contracted vertex in the next timestep. More concretely, we require $D_i^v$ to be a binary sequence of length $\widetilde{O}(w_{T_i}(v))$ for any vertex $v \in V_i$ at any timestep $i \geq 0$, and we wish any sequence of applications of contracting functions in $\mathcal{G}$ maintains this condition given that it is satisfied for its input vertices. In Definition~\ref{def:w-bounded} in Appendix~\ref{sec:further}, we formally define the \emph{$w$-bounded} property for a valid collection of contracting functions to address this restriction.

\fi

\begin{remark*}
It is worth mentioning that in \emph{proper binary trees}, binary trees in which every non-leaf vertex has degree $2$, it is possible to guarantee $O(\log{n})$ phases using only \rake s~\cite{kosaraju1988optimal}. In this variant of tree contraction, there is no \compress{} stage, and each \rake{} operation contracts a leaf along with its parent into its grandparent -- the parent of its parent. Although it is not hard to reduce a tree contraction on a general tree into an instance of tree contraction on proper binary trees for many problems, doing so will make the contracting functions more complicated, and the \degres{} property is not necessarily preserved.
\end{remark*}

% We will later show this algorithm can simulate $\alpha$-tree-contractions for any $2 \leq \alpha \leq n^\epsilon$. 


==> preorder.tex <==
%\section{Tree Contraction with Bounded Weights}\label{sec:bounded_weight}



\subsection{Generalized $\alpha$-Tree-Contractions}

In the rest of this section we prove Theorem~\ref{thm:main}. We assume that tree $T$ is already rooted at vertex $1$, and the vertices are already indexed by their preorder numbering. Otherwise, we may use Theorem 7 and Lemma 8.6 of Behnezhad et al.~\cite{behnezhad2019massively} respectively to make the tree rooted, and to find the preorder numbering of the vertices. Both algorithms require $O(n^\epsilon)$ memory per machine and $\widetilde{O}(n)$ total memory to finish in $O(1/\epsilon)$ AMPC rounds. 

Note that we only need to find the preorder numbering of $T$ once in the beginning. In order to find a \emph{preorder decomposition} at the beginning of each phase, we may sort the surviving vertices by their current preorder numbers, and then relabel them so that the vertices are numbered $1, 2, ..., |T_i|$. However, doing this requires $O(1/\epsilon)$ AMPC rounds during each phase~\cite{goodrich2011sorting}. Fortunately, it is possible to find an imperfect preorder numbering of vertices $0 < a_1 < a_2 < \ldots < a_k$ in $O(1)$ rounds so that $k = O(n^{1-i\epsilon})$. In Observation~\ref{obs:relabel}, we show how to find an imperfect preorder numbering of vertices at the beginning of each round.

\begin{observation}\label{obs:relabel}
It is possible to relabel the surviving vertices by a sequence $0 < a_1 < a_2 < \ldots < a_k$ at the beginning of round $i$, so that $k = O(n^{1-i\epsilon})$ and the associated vertices to $a_j$s for $1 \leq j \leq |T_i|$ are sorted by their actual preorder numbering.
\end{observation}

\begin{proof}
For the first case of Theorem~\ref{thm:bounded-weight} ($w(v) = 1$), we already know that at most one vertex survives in each part of a preorder decomposition of every $T_i$ due to \ref{lemma:preorder-decomposition}. Hence, we only need to divide the index of each vertex in the preorder traversal of $T_i$ by $n^\epsilon$ to find the preorder number of that vertex in $T_{i+1}$.

For the second case ($w(v) = \degr(v)$), we need to do a trick in order to relabel the surviving vertices in $O(1)$ AMPC rounds. Since the number of vertices in each partition are not equal in this case as we perform a weighted preorder decomposition, dividing the current preorder numbering may yield an invalid relabeling. To address this issue, we increase the current preorder number of each vertex in part $i$ by $in^\epsilon$ so that the division of every preorder number by $n^\epsilon$ produces distinct integers. This approach guarantees that the numbers associated with all vertices in $T_i$ are bounded by $2^{O(1/\epsilon)}|T_i| = O_{\epsilon}(|T_i|)$ after $O(1/\epsilon)$ phases and will always form a valid relabeling.
\end{proof}

The algorithm is explained in more details in the following. 
%You can also find more details in Algorithm~\ref{alg:w-bounded}.
There are three stages in each phase $i$:


\begin{enumerate}
    \item Find a preorder decomposition $V_1,V_2,\ldots,V_k$ of $T_{i-1}$ based on the given weight function $w_{T_{i-1}}:V\to\mathbb{Z}^{\geq0}$ and parameter $\lambda=n^\epsilon$.
    This step needs $O(1)$ rounds by reusing the existing preorder numbering of vertices to find the preorder numbering of $T_{i-1}$.
    \item For each connected component $C_{i,j}$ of each group $V_i$ apply the given Compress function $\C$ in parallel, i.e.,\[D_i^{C'_{i,j}} = \C(D_{i-1}^{C_{i,j}}) \quad \forall{i \in [k], j \in [c_i]}.\]
    According to Observation~\ref{obs:groups}, the total memory of the data stored on each $V_i$, and hence each $C_{i,j}$, is bounded by $O(n^\epsilon)$. Therefore, we can fit each group $V_i$ in a single machine and perform this stage locally. Then, let $T_i = T'_{i-1}$ where $T'_{i-1}$ is the dependency tree of $T_{i-1}$.
    \item Reduce the number of leaves in $T_i$ to $O(k)$.
    We could potentially have $\omega(k)$ remaining leaves after compressing all $C_{i,j}$'s while the number of non-leaves, i.e., \emph{dependent subtrees}, is bounded by $O(k)$ due to Lemma~\ref{lemma:preorder-decomposition}. The number of groups $k$ is in turn bounded by $O(n^{1-i\epsilon})$ if $w(v) \leq n^\epsilon$ for all $v \in V$ due to Observation~\ref{obs:groups}. 
If we also reduce the number of leaves in the tree to $O(k)$, the number of remaining vertices drops to $O(n^{1-i\epsilon})$ at the end of phase $i$. For two cases of Theorem~\ref{thm:bounded-weight}, $w(v) = 1$ and $w(v) = \degr(v)$, we use the given Rake function $\R$ in two different ways to achieve this step.
\end{enumerate}


To finish the algorithm, after $l = O(1/\epsilon)$ phases, we store the remaining graph, which contains at most $O(n^\epsilon)$ vertices, on one machine and compute $f(T_l)$ locally. 

We need to ensure $w(v) \leq \lambda  = n^\epsilon\;\;\forall{v \in V}$ throughout the algorithm so that the first stage successfully finds a preorder decomposition of $T_{i-1}$. This frameworks depends on the fact that $\mathcal{G} = \{ \C, \R \}$ is $w$-bounded since we need to merge the partial solutions computed in the second stage efficiently, and the memory needed to store the contracted data needs to be somehow bounded. This memory constraint is the main property of a $w$-bounded $\mathcal{G} = \{ \C, \R \}$ defined in Definition~\ref{def:w-bounded}, and it guarantees that the $w(v) \leq \lambda$ holds after any sequence of contractions.


%\hamed{The weight function also needs to have the property that $w_{T'}(S') \leq w_T(S) = \sum_{v \in S}{w_T(v)} \;\;\forall{S \subseteq T}$. This property implies that at no stage in the algorithm $w(v)$ surpasses $n^\epsilon$ at any stage of the algorithm, not only the beginning.}


%\hamed{We need to take care about this step when $w(v)$ is not equal to the number of children of $v$. As we might have more than $n^\epsilon$ leaves in each leaf-star. Probably requiring another semi-contracting function which reduces the number of leaves without changing the data of the parent.}


%In the following theorem, we argue that Algorithm~\ref{alg:w-bounded} computes any $w$-bounded function $f(T)$ in $O(1/\epsilon)$ AMPC rounds as long as $w(v) \leq n^\epsilon \;\;\forall{v\in V}$.

%To prove correctness of the algorithm, we need to address two things: (1) the remaining graph fits on one machine after $O(1/\epsilon)$ phases and (2) each phase is implementable in $O(1)$ AMPC rounds.

%(1) Consider phase $j$ of the algorithm on a connected subgraph of $T_{j-1}$. According to Lemma~\ref{lemma:preorder-decomposition}, each group $V_i$ has at most one dependent subtree, which we denote by $C_{i,c_i}$ wlog. Each independent subtree in $V_i$, subtress $C_{i,1}, \ldots, C_{i,c_i-1}$, is a leaf in $T_j = T'_{j-1}$ according to the definition. Since $T_j$ has at most $k$ non-leaf vertices and at most $\widetilde{O}(k)$ leaves after shrinking the \emph{leaf-star}s, and the fact that $k$ is at most a $O(1/n^\epsilon)$ fraction of the number of remaining vertices due to Observation~\ref{obs:groups}, the number of the remaining vertices drops by a factor of $O(n^\epsilon)$ in $T_j$. Hence after $l = O(1/\epsilon)$ phases, the remaining tree $T_l$ has at most $O(n^\epsilon)$ vertices and fits into a single machine. 
%Independent leaf subtrees may end up isolated (and thus removed) as well if their parents are matched. Also, the only vertex that remains in $C_{i,1}$ is the last vertex, vertex with index $l_i$. 
%All non-leaf vertices are matched, according to the definition of the greedy algorithm in the third stage, and unmatched leaves of $C_{i,1}$ are isolated unless they are the last vertex, due to basic properties of the preorder numbering. 
%This implies the only vertices remaining after phase $j$ are either independent leaf subtrees or the last vertex in $C_{i,1}$ for $i \in [k]$, which is also the last vertex of the group or $l_i$. 

%(2) To can greedily find a preorder decomposition $V_1, V_2, \ldots, V_k$ of $T_{j-1}$ in step $j$ due to Observation~\ref{obs:groups}. Since the vertices are already sorted based on their preorder numbering, we can easily implement the first stage in $O(1)$ MPC rounds by keeping track of partial sum of the weights. Then, we send each group to an individual machine.
%Then, we locally find the connected components of each group $V_i$, i.e., $C_{i,1}, C_{i,2}, \ldots, C_{i,c_i}$, and perform the $w$-bounded function $f$ on each component $C_{i,j}$. Thus, the second stage is done entirely local and needs no communication rounds. %\hamed{Shrinking leaf-stars is tricky!}

% We would like to remark that although we assumed $\R$ is a connected contracting function, Theorem~\ref{thm:bounded-weight} also works with a sibling contracting Rake function. Additionally, one can easily observe than $F^{\R}(n) = O(1/\epsilon)$ for any sibling contracting function $\R$. In the rest of this section, we improve the round complexity of Theorem~\ref{thm:bounded-weight} potentially from $O(1/\epsilon^2)$ to $O(1/\epsilon)$ when we are given a \emph{sibling contracting} Rake function $\R$. 

% By utilizing \textsf{SiblingReduceLeaves} in the third stage of each phase, the second case of Theorem~\ref{thm:bounded-weight} where $w(v) = 1$ is implied. 
 
%First, in Lemma~\ref{lemma:sibling-w1}, we claim that every $w$-bounded collection $\mathcal{G}$ containing at least one sibling contracting function must satisfy $w(v) = 1$. 



Due to Observation~\ref{obs:relabel}, it is possible to implement the first two stages of the algorithm in $O(1)$ AMPC rounds. Thus, the round complexity of the algorithm depends only on the way we implement the third stage. A natural way to achieve this is to aggregate the data stored on all \emph{leaf-star}s in $T_i$ by applying the contracting Rake function $\R$.
Consider a leaf-star $S = \{ v_1, v_2, \ldots, v_k \}$ with the common parent $u$. In the first case of Theorem~\ref{thm:bounded-weight}, the size of each leaf-star is bounded by $O(n^\epsilon)$ since we have $w(v) = \degr(v) \leq n^\epsilon$ throughout the algorithm. 
The degree $w(v)$ of each vertex $v \in T_i$, in each phase $i$, is bounded by $n^\epsilon$ since Observation~\ref{obs:groups} ensures that the total weight, and consequently the total degree, of the vertices in each part of preorder decomposition is bounded $O(n^\epsilon)$. Therefore, the degree of any contracted vertex is also bounded by $O(n^\epsilon)$.
    %We assume R is a connected contracting function in this case althoguh it also works if we have a sibling contracting function instead
    We assume $\R$ is a connected contracting function in this case although it also works if we have a sibling contracting function instead.
    Apply $\R$ on the connected component induced by $S_* = \{ u, v_1, v_2, \ldots, v_k \}$:\[D_i^{S_{*}'} = \R(D_{i-1}^{S_*}).\]
    % Depending on the type of the contracting function $\R$, we apply it differently:
    %\begin{itemize}
    %    \item Given a \emph{connected contracting} Rake function $\R$, we apply $\R$ on the connected component induced by $S_* = \{ u, v_1, v_2, \ldots, v_k \}$:\[D_i^{S_{*}'} = \R(D_{i-1}^{S_*}).\]
    %    \item Given a \emph{sibling contracting} Rake function $\R$, we apply $\R$ on $S$: \[D_i^{S'} = \R(D_{i-1}^S).\]
    %\end{itemize}
    See Algorithm~\ref{alg:connected-rake} for formal definition of the \textsf{ReduceLeaves} subroutine we use in this case.
    After applying $\R$ on all leaf-stars, at most one leaf remains for each leaf-star (Note that the parent itself becomes a leaf). Thus, the number of leaves is reduced to $O(k)$.
    % This implies that the number of remaining vertices is bounded by $O(n^{1-\epsilon})$ according to Lemma~\ref{lemma:preorder-decomposition}. This step needs $O(F^{\R}(n))$ AMPC rounds, assuming applying $\R$ on a leaf-star of size $O(n)$ takes $F^{\R}(n)$ rounds. We will later improve this stage to avoid dependence on $O(F^{\R}(n))$ if we are given a \emph{sibling contraction} Rake function.
    
    
\begin{algorithm}[ht]
\SetAlgoLined
\KwData{Tree $T$ and a \emph{connected contracting} Rake function $\R$.}
\KwResult{Tree $T$ with reduced leaves.}
Let $\mathcal{L}$ be the set of all maximal leaf-stars in $T$\;
 \For{$S = \{ v_1, v_2, \ldots, v_k \} \in\mathcal{L}$}{
    $S_* \leftarrow S \cup(u)$ where $u$ is the common parent of all leaves in $S$\;
    Contract $S_*$ by applying $D_{i+1}^{u} = \R(D_i^{S_*})$\;
  }
 \caption{\textsf{ConnectedReduceLeaves} \\ (\textsf{ReduceLeaves} subroutine when $w(v) = \degr(v) \leq n^\epsilon$)}
\label{alg:connected-rake}
\end{algorithm}

To address the second case of Theorem~\ref{thm:bounded-weight}, where $w(v) = 1$, we give an alternative \textsf{ReduceLeaves} subroutine for the third stage of the algorithm. We present this subroutine in Algorithm~\ref{alg:sibling-rake}, and we prove that it works in Lemma~\ref{lemma:sibling-reduce}. Note that an example problem \textsf{SumParent}, in which there are some values on the leaves and value $f(v)$ of an internal vertex $v$ is recursively defined as the sum of the value of its children, there exists a $w$-bounded collection of contracting functions $\mathcal{G} = \{ \C, \R \}$ with $w(v) = 1$ such that $\R$ is a sibling contracting function. Using Algorithm~\ref{alg:connected-rake} in the third stage of algorithm gives us an $O(1/\epsilon^2)$ rounds AMPC algorithm for this problem since raking a leaf-star of size $O(n)$ needs $O(1/\epsilon)$ rounds\footnote{For a leaf-star $S$, apply $\R$ based on a balanced $n^\epsilon$-ary tree whose leaves are the elements of $S$.}. Yet we improve the total round complexity to $O(1/\epsilon)$ by utilizing Algorithm~\ref{alg:sibling-rake} in the third stage of the algorithm.

\begin{algorithm}[ht]
\SetAlgoLined
\KwData{Tree $T$, a preorder decomposition $V_1, V_2, \ldots, V_k$, and a \emph{sibling contracting} Rake function $\R$.}
\KwResult{Tree $T$ with reduced leaves.}
Let $\mathcal{L}_i$ be the set of all maximal leaf-stars in $V_i$ for all $i \in [k]$\;
 \For{$S = \{ v_1, v_2, \ldots, v_k \}\in\cup_{i=1}^{k}{\mathcal{L}_i}$}{
    Aggregate the data stored on $S$ by applying $D_{i+1}^{v_1} = \R(D_i^S)$\;
  }
 \caption{\textsf{SiblingReduceLeaves} \\ 
  (\textsf{ReduceLeaves} subroutine when $w(v) = 1$)}
\label{alg:sibling-rake}
\end{algorithm}


%\begin{lemma}\label{lemma:sibling-w1}
%A valid collection of contracting functions $\mathcal{G} = \{ g_1, g_2, \ldots, g_l\}$ which contains at least one \emph{sibling contracting} function is $w$-bounded only if $w(v) = \widetilde{O}(1)$ for all $v \in V$.
%\end{lemma}
%\begin{proof}
%Assume by contradiction that $|D_0^v| = \Theta(w(v)) = \widetilde{\omega}(1)$ for some vertex $v \in V$. Let $u_1, u_2, \ldots, u_k$ be the children of $v$ in $T_0$. Recall that there exists at least one connected contracting function $g_j$ in any valid collection of contracting functions $\mathcal{G}$. By applying $g_j$ on the subtree rooted at every $u_i$ at timestep $0$, $S = \{ u_1, u_2, \ldots, u_k \}$ becomes a leaf-star in $T_1$. This means that $|D_1^{u_i}| = \widetilde{O}(1)$ for any $i \in [k]$. 

%Next, apply a sibling contraction function $g_z \in \mathcal{G}$  on leaf-star $S = \{ u_1, u_2, \ldots, u_k \}$ to aggregate the data $(D_1^{u_1}, D_1^{u_2}, \ldots, D_1^{u_k})$ into a single data entry $D_2^{u_1}$. Since $u_1$ is now the only child of $v$ and $\degr_{T_2}(v) = 1$, then the length of $D_2^{v}$ must be at most $\widetilde{O}(1)$ according to the definition of $w$-bounded. However, no contracting function is applied on $v$ up to timestep $2$, hence $D_2^v = D_0^v$. This contradicts our assumption that $|D_0^v| = \widetilde{\omega}(1)$.
%\end{proof}


\begin{lemma}\label{lemma:sibling-reduce}
The number of leaves in $T_i$ reduces to $O(k)$ if we use \textsf{SiblingReduceLeaves}, defined in Algorithm~\ref{alg:sibling-rake} in the third stage of the algorithm.
\end{lemma}
\begin{proof}
We allocate two tokens for each group $V_j$ for a total of $2k$ tokens. Denote the first and the second token of group $V_j$ by $A_j$ and $B_j$ respectively. Consider a leaf-star $S = \{u_1, u_2, \ldots, u_k\}$ so that $v$ is the common parent of the leaves in $S$. Let $v \in V_{j_0}$, and $\{ V_{j_1}, V_{j_2}, \ldots, V_{j_l} \}$ be the set of groups which leaves in $S$ belong to, such that $j_0 < j_1 < \ldots < j_l$. Thus, $l$ leaves remain connected to $v$ after running \textsf{SiblingReduceLeaves} on $T_i$, say $u'_1, u'_2, \ldots, u'_l$ so that $u'_{i'} \in V_{j_{i'}}$. Use token $A_{j_0}$ for $u'_{j_l}$, and use token $B_{j_{i'}}$ for each $u'_{j_{i'}}$ for each $1 \leq i < l$.

First, we claim that each token $A_j$ is used at most once. According to Lemma~\ref{lemma:preorder-decomposition}, each group $V_j$ has at most one non-leaf vertex in the dependency tree $T'_{i-1}$, and consequently in $T_i$. Therefore, there is at most one leaf-star with parent $v \in V_j$, and token $A_j$ is used at most once in that leaf-star.

Second, we claim that each token $B_j$ is used at most once. Whenever we use token $B_j$ for some leaf $u \in V_j$, there exists another leaf $u' \in V_{j'}$ in the same leaf-star as $u$ such that $j < j'$. According to the basic properties of preorder numbering, this leaf-star is the leaf-star with highest-indexed parent which contains a leaf from group $V_j$. Thus, we use token $B_j$ of group $V_j$ in at most one leaf-star. Lemma~\ref{lemma:sibling-reduce} statement is implied.
\end{proof}

%\boundedweightsibling*


==> treecontraction.tex <==
\section{Generalized Tree Contraction}\label{sec:main}

%\emph{Tree Contraction} is originally introduced by Miller and Reif~\cite{miller1989parallel}. Given two \emph{valid contracting functions} $\C$ and $\R$ as a black-box, it is possible to compute a global property about a tree in $O(\log{n})$ phases.
%In each phase, we have two stages: \compress{} and \rake{}. In a \compress{} stage, we contract around half the vertices with only one child into their parent using $\C$, and in a \rake{} stage, we contract all the leaves in the remaining tree into their parent using $\R$. 

%In the original variant, every odd-indexed vertex in each \emph{chain}, a maximal connected sequence of vertices each with only one child, is removed in a \compress{} stage. In some randomized variants, each vertex is selected with probability $1/2$ independently, and an independent set of the selected vertices is contracted. We consider a more relaxed variant of the \compress{} stage where each maximal chain is contracted into a much smaller number of  vertices, or even one, by performing a \compress{} stage. For example, assume the number of vertices in each chain drops by a factor of $O(n^\epsilon)$ in one \compress{} stage. In all of these variants, repeating \compress{} and \rake{} stages alternatively $O(\log(n))$ times results in a single remaining vertex.

%We can define a more general version of tree contraction as follows: In \emph{$\alpha$-tree-contraction} the \rake{} stage is the same as before, but in the \compress{} stage every maximal subgraph containing only vertices with degree less than $\alpha$ is contracted into a single vertex. According to this definition, typical tree contraction is equivalent to $2$-tree-contraction. Note that we assume a variant of tree contraction in which every chain is contracted into a smaller number of vertices in each \compress{} stage. 

%\begin{definition}\label{def:alpha-tc}
%In an $\alpha$-tree-contraction of a tree $T=(V,E)$, we repeat two stages in a number of phases until the whole tree is contracted into a single vertex:
%\begin{itemize}
%    \item \compress{} stage: Contract every maximal connected component $S$ containing only vertices with degree less than $\alpha$, i.e., $\degr(v)\leq \alpha\;\;\forall{v \in S}$, into a single vertex $S'$.
%    \item \rake{} stage: Contract all the leaves into their parent.
%\end{itemize}
%\end{definition}

%Interestingly, it is possible to solve a broad range of DP formulation on trees in $O(1/\epsilon^2)$ AMPC rounds using $n^\epsilon$-tree-contraction. 
% \hamed{Ref to max matching as an example} 
%Similar to the fact that the number of tree contraction rounds, i.e. performing a \compress{} stage and a \rake{} stage on the remaining tree, is bounded by $O(\log(n))$ in $2$-tree-contraction, we show an upper bound of $O(1/\epsilon)$ for the number of tree contraction rounds in $n^\epsilon$-tree-contraction. More generally, we provide an upper bound for $\alpha$-tree-contraction in the following lemma.
In this section, we demonstrate our main result (Theorem~\ref{thm:main}) which allows us to compute a global property of a tree $T$, which admits $w$-bounded collection of contracting functions, using $\alpha$-tree-contraction in $O(1/\epsilon^2)$ AMPC rounds. Recall the definition of $\alpha$-tree-contraction (Definition~\ref{def:alpha-tc}) from Section~\ref{subsec:generalized-tree-contraction}. First, we prove Lemma~\ref{lemma:rounds} to bound the number of phases in $\alpha$-tree-contraction.

% Using Lemma \ref{lemma:rounds}, we aim to compute a function $f(T)$ defined on a tree in $O(1/\epsilon^2)$ AMPC rounds using $n^\epsilon$-tree-contraction, as long as we can guarantee that the size of the data stored in each vertex is proportional to the number of its children in the contracted graph. More precisely, we need to show that contracting a maximal connected component $S$ containing only low-degree vertices, with less than $\alpha$ children, is possible so that it takes $O(1/\epsilon)$ AMPC rounds, and the output fits into a $O(\degr_{T'}(S'))$ memory, where $\degr_{T'}(S')$ is the number of the degree of the contracted vertex $S'$ in the contracted tree $T'$. 

\marina{I think I stole this lemma and moved it when I shouldn't. Not sure it belongs here but you can check the DISC submission to see}
\begin{lemma}\label{lem:rounds}
For any $\alpha \geq 2$, the number of $\alpha$-tree-contraction phases until we have a constant number of vertices is bounded by $O(\log_{\alpha}(n))$.
\end{lemma}

\marina{What happened to this theorem?}
\alpharounds*

To show Lemma~\ref{lemma:rounds} we will introduce a few definitions. The first definition we use is a useful way to represent the resulting tree after each \compress{} stage. Before stating the definition, recall the \emph{Dependency Tree} $T'$ of a tree $T$ from Definition~\ref{def:dependency-tree}.

\begin{definition}
An \textbf{$\alpha$-Big-Small Tree} $T'$ is the \emph{dependency tree} of a tree $T$ with weighted vertices if it is a minor of $T$ constructed by contracting all components of $T$ made up of vertices $v$ with $w_T(v) \leq \alpha$ (i.e., the connected components of $T$ if we were to simply remove all vertices $u$ with $w_T(u) > \alpha$) into a single point.

We call a node $v$ in $T'$ that was of weight $w_T(v) > \alpha$ in $T$ a \textbf{big node}. All other nodes in $T'$, which really represent contracted components of small vertices in $T$, are called \textbf{small components}. 
\end{definition}

Note that a small component may not be small in itself, but it can be broken down into smaller vertices in $T$. It is not hard to see the following simple property. This simply comes from the fact that maximal components of small degree vertices are compressed into a single small component, thus no two small components can be adjacent.

\begin{observation}\label{obs:bigsmall}
No small component in an \bigsmall{} can be the parent of another small component.
\end{observation}

Consider our dependency tree $T'$ based off a tree $T$ that has been compressed. Obviously, $T'$ is a minor of $T$ constructed as described for $\alpha$-Big-Small Tree because the weight of a vertex equals its number of children (by the assumption of Lemma~\ref{lemma:rounds}). Note a small component refers to the compressed components, and a big node refers to nodes that were left uncompressed. %In order to use this in our proofs, we will define one more convenient term:

To show Lemma~\ref{lemma:rounds}, we start by proving that the ratio of leaves to nodes in $T'$ is large. Since \rake{} removes all of these leaves, this shows that $T$ gets significantly smaller at each step. Showing that the graph shrinks sufficiently at each phase will ultimately give us that the algorithm terminates in a small number of phases.

\begin{lemma}\label{lemma:reduceverts}
Let $T_i'$ be the tree at the end of phase $i$. Then the fraction of nodes that are leaves in $T_i'$ is at least $\alpha/(\alpha+4)$ as long as $w(v)$ is equal to the number of children of $v$ for all $v\in T_i'$ and $\alpha \geq 2$.
\end{lemma}


\begin{proof}
For our tree $T_i'$, we will call the number of nodes $n$, the number of leaves $\ell$, and the number of big nodes $b$. We want to show that $\ell > n\alpha/(\alpha+4)$. We induct on $b$. When $b=0$, we can have one small component in our tree, but no others can be added by Observation~\ref{obs:bigsmall}. Then $n=\ell=1$, so $\ell> n\alpha/(\alpha+4)$. \hamed{inspect +4}

Now consider $T_i'$ has some arbitrary $b$ number of big nodes. Since $T_i'$ is a tree, there must be some big node $v$ that has no big node descendants. Since all of its children must be small components and they cannot have big node descendants transitively, then Observation~\ref{obs:bigsmall} tells us each child of $v$ is a leaf. Note that since $v$ is a big node, it must have weight $w(v) > \alpha$, which also means it must have at least $\alpha$ children (who are all leaves) by the assumption that $w(v)$ is equal to the number of children.

Consider trimming $T_i'$ on the edge just above $v$. The size of this new graph is now $n^* = n - w(v) - 1$. It also has exactly one less big node than $T_i'$.  Therefore, inductively, we know the number of leaves in this new graph is at least $\ell^* \geq \frac{\alpha}{\alpha+4}n^* = \frac{\alpha}{\alpha+4}(n-w(v)-1)$. Compare this to the original tree $T_i'$. When we replace $v$ in the graph, we remove up to one leaf (the parent $p$ of $v$, if $p$ was a leaf when we cut $v$), but we add $w(v)$ new leaves. This means the number of leaves in $T_i'$ is:
\begin{align*}
\ell =& \ell^* - 1 + w(v)
\\=& \frac{\alpha}{\alpha+4}(n-w(v)-1) - 1 + w(v)
\\=& \frac{\alpha}{\alpha+4}n - \frac{\alpha}{\alpha+4}w(v) - \frac{\alpha}{\alpha+4} - 1 + w(v)
\\=& \frac{\alpha}{\alpha+4}n + \frac{4}{\alpha+4}w(v) - \frac{2\alpha+4}{\alpha+4}
\\>& \frac{\alpha}{\alpha+4}n + \frac{4}{\alpha+4}\alpha - \frac{2\alpha+4}{\alpha+4}\tag{1}\label{line:big}
\\\geq& \frac{\alpha}{\alpha+4}n\tag{2}\label{line:alpha}
\end{align*}

Where in line~(\ref{line:big}) we use that $w(v) > \alpha$ and in line~(\ref{line:alpha}) we use that $\alpha \geq 2$.
\end{proof}

Now we can prove our lemma.

\begin{proof}[Proof of Lemma~\ref{lemma:rounds}]
To show this, we will prove that the number of nodes from the start of one \compress{} to the next is reduced significantly. Consider $T_i$ as the tree before the $i$th \compress{} and $T_i'$ as the tree just after.  Let $T_{i+1}$ be the tree just before the $i+1$st \compress, and let $n_i$ be the number of nodes in $T_i$, $n_i'$ be the number of nodes in $T_i'$, and $n_{i+1}$ be the number of nodes in $T_{i+1}$. Since $T_i'$ is a minor of $T_i$, it must have at most the same number of vertices as $T_i$, so $n_i'\leq n_i$. Since $T_{i+1}$ is formed by applying \rake{} to $T_i'$, then it must have the number of nodes in $T_i'$ minus the number of leaves in $T_i'$ ($\ell_i'$). Therefore:

\[n_{i+1} = n_i' - \ell_i' \leq n_i' - \frac{\alpha}{\alpha+4}n_i' = \frac4{\alpha+4}n_i' \leq \frac4{\alpha+4}n_i\]

Where we apply both Lemma~\ref{lemma:reduceverts} that says $\ell_i' \geq \frac\alpha{\alpha+4}n_i'$ and the fact that we just showed that $n_i'\leq n_i$. This shows that from the start of one compress phase to another, the number of vertices reduces by a factor of $\frac4{\alpha+4}$. Therefore, to get to a constant number of vertices, we require $\log_{\frac{\alpha+4}{4}}(n) = O(\log_\alpha(n))$ phases.

\end{proof}

%\begin{definition}
%We say a node in some $\alpha$-Big-Small tree $T$ is \textbf{a small leaf component} if it is a small component that is a leaf.
%\end{definition}

\iffalse
\begin{definition}
We say a node in some $\alpha$-Big-Small tree is \textbf{bad} if it has at least $\alpha$ non-leaf children.
\end{definition}



\begin{proof}
If we can show that the total weight of the tree is reduced by a factor of $\alpha$ each phase, then in $O(\log_\alpha(n))$ phases, we will have constant weight and thus have completed the algorithm. Specifically, we will show that from the start of one \compress{} stage to the start of the \compress{} stage in the next phase, the tree weight is reduced by a factor of $\alpha$. To see why, fix some phase $i$. Let $T_i$ and $T_i'$ be the trees just before and after the $i$th \compress{} respectively. As described previously, $T_i'$ is an $\alpha$-Big-Small tree.

Next, consider the following transformation: let $T_i^*$ be obtained by contracting all small components in $T_i'$ with their parent. This is quite similar to how \rake{} will work in the next step, but it also contracts internal small components with their parents. Note that small components cannot be parents to other small components, otherwise they would be parts of the same small component. Therefore, we are merging small components with their big node parents. We will refer to these joined vertices by the name of the big node parent. Note there $T_i^*$ has one vertex for every big node in $T_i'$ and preserves the structure of dependencies between them.

Consider $v$, a bad vertex in $T_i'$. Consider a child $u$ of $v$ that has no big node descendant. Then the entire tree at and below $u$ in the original tree $T_i$ would necessarily consist of nodes with small weight, and thus small degree. Therefore, the entire tree at and below $u$ would form a single small component in $T_i'$. Therefore, since $v$ is a bad vertex, it must have more than $\alpha$ children that have at least one big node descendant. This means $v$ has at least $\alpha$ children in $T_i^*$. 

Assume for contradiction that more than a $1/\alpha$ fraction of big vertices in $T_i'$ are bad. Since $|T_i^*|$ is the number of big vertices in $T_i'$, this implies that the number of bad vertices is $b > |T_i^*|/\alpha$. Let's count the number of edges in $T_i^*$ (which is the same as $|T_i^*|-1$) by counting the number of outgoing edges (i.e., edges to children) from each vertex. The number of outgoing edges due to each bad vertex is at least $\alpha$, so the total number of outgoing edges due to bad vertices is at least  $\alpha b > |T_i^*|$. This contradicts that we have $|T_i^*|$ edges in the tree. Therefore, at most $1/\alpha$ of the big vertices in $T_i'$ are bad.

This is sufficient set up to consider the change in weight of the trees. Consider again $T_i$ before the $i$th \compress{} and $T_i'$ just after. Then $T_{i+1}$ builds on top of $T_i'$ by running the \rake{} function. Recall that we assume that at all times, the weight of a vertex is its number of children. That means the total weight corresponds to the total number of children across all nodes, or, the number of edges in the graph. This is bounded above by the number of vertices in $T_{i+1}$.

To bound the number of nodes in $T_{i+1}$, consider that \rake{} will trim all leaves from the graph. In \compress{} we compressed each leaf in $T_i'$ into a single vertex, which was notably a leaf. Therefore all such components were removed in constructing $T_{i+1}$. For every big node in $T_i'$, we know that all but at most 

consider how we showed that only one compressed vertex is created for each group in the preprocessing. Since each group covered $n^\epsilon$ distinct vertices in $T$, there were at most $n^{1-\epsilon}$ groups, and thus compressed vertices. Therefore, $|T_0| \leq n^{1-\epsilon}$. Therefore, the weight across all nodes in $T_0$ is bounded above by $n^{1-\epsilon}$.

Now we must show this extends to $T_i$. The difference between $T_0$ and $T_i$ is only what occurs during the phases. During phases, all we do is solve and contract small components and big nodes in the previous tree, updating weights as we go. Therefore, the total weight can only get lower. This means the total weight of $T_i$ is bounded above by $n^{1-\epsilon}$.

Finally, since $T_v$ is a subtree of $T_i$, the weight of $T_v$, too, is bounded above by $n^{1-\epsilon}$.
\end{proof}
\fi

Using Lemma \ref{lemma:rounds}, we aim to compute a function $f(T)$ defined on a tree in $O(1/\epsilon^2)$ AMPC rounds using $n^\epsilon$-tree-contraction, as long as we can guarantee that the size of the data stored in each vertex is proportional to the number of its children in the contracted graph. More precisely, we need to show that contracting a maximal connected component $S$ containing only low-degree vertices, with less than $\alpha$ children, is possible so that it takes $O(1/\epsilon)$ AMPC rounds, and the output fits into a $O(\degr_{T'}(S'))$ memory, where $\degr_{T'}(S')$ is the number of the degree of the contracted vertex $S'$ in the contracted tree $T'$. 

We require a $w$-bounded collection of contracting functions $\mathcal{G} = \{ \C, \R \}$ so that $w(v) = \degr(v)$ for all $v \in V$, where $\R$ is a sibling contracting Rake function. 
% <new>
We then utilize the first case of Theorem~\ref{thm:bounded-weight} with $\mathcal{G} = \{ \C \}$ as a blackbox to contract the maximal connected components of low-degree vertices in each \compress{} stage. Note that we pass only $\C$ as both Rake and Compress functions to Theorem~\ref{thm:bounded-weight} since we practically compress a connected component of size at most $O(n^\epsilon)$ in \textsf{ConnectedReduceLeaves} subroutine (Algorithm~\ref{alg:connected-rake}) which can be done using $\C$, and it is the only place that we use the contracting Rake function in Theorem~\ref{thm:bounded-weight} given that $w(v) = \degr(v) \leq n^\epsilon$. However, we still use a sibling contracting function $\R$ in the \rake{} stage of our algorithm in this section.
% </new>

%\hamed{I don't get the following} Note that we can perform \blackbox{Rake} steps using the same function $R$ we used for $2$-tree-contraction. 
%In other words, a DP formulation on a tree can be solved in $O(1/\epsilon)$ AMPC rounds if we are given a black-box function $C$ which maintains the mentioned memory constraints in a \blackbox{Compress} stage.

%\begin{definition}
%\hamed{Redundant, covered by $w$-bounded}
%We say a black-box function, either \blackbox{Rake} or \blackbox{Compress}, is a \emph{well-behaved} black-box function if its output size\footnote{The output of both functions is the data we store in the contracted vertex $v$, and the output of the whole problem is the data we store in root when the tree contraction process is finished.} is bounded by $\tilde{O}(d_v)$, where $d_v$ is the number of children of a contracted vertex $v$. 

%\begin{itemize}
%    \item The \blackbox{Rake} function contracts a number of sibling leaves into their parent.
%    \item The \blackbox{Compress} function contracts a number of vertices with low degree, less than $\alpha$,  into a vertex representing this component.
%\end{itemize}
%\end{definition}

\main*

\begin{proof}
We will show that our Algorithm~\ref{alg:main}, where notably $\alpha=n^\epsilon$, achieves this result. Lemma~\ref{lemma:rounds} shows that there will be only at most $O(1/\epsilon)$ phases. In each phase, we start by running a connectivity algorithm to find maximally connected components of bounded degree, which takes $O(1/\epsilon)$ time. Then for each component $C_j$ which is a leaf in $T'_i$, we run \textsf{BoundedTreeContract} (Algorithm~\ref{alg:w-bounded}),
%\hamed{I'm not sure where the fact that we only compress leaves is used in this proof. But I guess it affects Lemma~\ref{lemma:reduceverts}. We also need to define $\mathcal{K}$.}  
using only our compressor function, i.e, $\mathcal{G} = \{ \mathcal{C} \}$, in parallel. Let $\mathcal{K}$ be the set of connected components which are leaves in $T'_{i-1}$. Since $\sum_{C_j} w(C_j) = w(T_i)$ for current tree $T_i$, the total number of machines is bounded above by $O(n^{1-\epsilon})$. By definition, the maximum degree of any $C_j$ is $n^\epsilon$. By Theorem~\ref{thm:bounded-weight}, each instance of \textsf{BoundedTreeContract} requires $O(1/\epsilon)$ rounds, $O(w(C_j)^\epsilon)$ local memory and $\widetilde{O}(w(C_j))$ total memory on its component $C_j$. As $w(C_j) \leq w(T_i)$ (we know $w(T_0) = O(n)$ and it only decreases over time), we only require at most $O(n^\epsilon)$ memory per machine. Since $\sum_{C_j} w(C_j) = w(T_i)$, the total memory required is only $\widetilde{O}(w(T_i)) = \widetilde{O}(n)$. This is within the desired total memory constraints.

Finally, $\mathcal{R}$ is given to us as a sibling contractor. Consider the \rake{} stage in our algorithm. We distribute machines across leaf-stars. For any leaf-star with $n^\epsilon \leq \degr(v) \leq kn^\epsilon$ for some (possibly not constant) $k$, we will allocate $k$ machines to that vertex. Since again the number of vertices is bounded above by $n$, this requires only $O(n^{1-\epsilon})$ machines. On each machine, we allocate up to $n^\epsilon$ leaf-children to contract into each other. We can then contract siblings into single vertices using $\mathcal{R}$. Since there are at most $n$ children for a single vertex, it takes at most $O(1/\epsilon)$ rounds to contract all siblings into each other. Then, finally, we can use $\mathcal{C}$ to compress the single child into its parent, which takes constant time.

Therefore, we have $O(1/\epsilon)$ phases which require $O(1/\epsilon)$ rounds each, so the total number of rounds is at most $O(1/\epsilon^2)$. We have also showed that throughout the algorithm, we maintain $O(n^\epsilon)$ memory per machine and $\widetilde{O}(n)$ total memory. This concludes the proof.
\end{proof}

\iffalse
The algorithm is described with an initial preprocessing step and then a process that occurs in \textit{phases}. The goal of each phase is to contract and trim the graph until it is small enough to fit on one machine. We will show that we only require $O(1/\epsilon)$ phases until this happens. Let $T_i$ be the tree at the beginning of phase $i$, where $T_0$ is a transformed, vertex-weighted version of $T$ based off a preprocessing step.

For the preprocessing step, the high level goal is to delay handling nodes with too many dependencies. This is because, as we showed in the last section, components with few dependencies can be compressed into smaller representations. To do this, we create the $n^\epsilon$-Big-Small graph of $T$. This can be done by running a breadth-first-search on at most $n$ nodes in $O(1/\epsilon)$ rounds and ignoring edges to vertices $v$ with weight $w(v) > n^\epsilon$. This only occurs once, at the start of the algorithm, and we will work on top of this starting tree $T_0$.

The next part of the algorithm will occur in phases. The basic idea of each phase it to select parts of the tree to solve entirely such that we can compress big nodes into $n^\epsilon$ size or smaller. Fix some phase $i$, and consider all big nodes in $T_0$. A big node will be compressible in this round if it has at most $n^\epsilon$ children that are \textit{not} small leaf components. We will later show that a large fraction of big nodes are compressible in this way.

In parallel, for all big nodes that will be compressible this phase, in parallel, we solve each of their small leaf component children. This will be done by decomposing the tree into groups and compressing connected components within each group iteratively. We describe this process below. Once we can solve each of the small leaf component children, we use the compression from Theorem~\ref{thm:compress} to write each of these big nodes in terms of their $n^\epsilon$ or fewer unknown children. Now they are small nodes. We are left with a tree of big nodes, small nodes, and small components. We then run a similar connectivity algorithm to join small components and small nodes to make our tree a valid $n^\epsilon$-Big-Small Tree again. Then we move on to the next phase.

The iterative decomposition and compression process is as follows (note that the max number of children a vertex will have at any time is $n^\epsilon$, we will show this later):

\begin{enumerate}
    \item First, we compute the pre-order numbering of vertices of $T$, but the pre-ordering is weighted in that a vertex $v$ with weight $w(v)$ counts as $w(v)$ many vertices $\{u_i^v\}_{i\in[w(v)]}$, and the pre-order number of $v$ is equal to the pre-order number of its first vertex $u_0^v$. Then, we will put all vertices $v$ with pre-order number at most $n^\epsilon$ in the first group, those with pre-order number between $n^\epsilon$ and $2n^\epsilon$ in the second group, and so on. Creating a pre-order numbering requires $O(1/\epsilon)$ AMPC rounds, and labeling the groups takes 1 round.
    \item Note that the total compressed size of a group is at most the total weight of the group, or $n^\epsilon$ plus the compressed size of the last vertex in the group. We assume that the compressed size of a vertex is at most $n^\epsilon$, this assumption will be clear later. Thus the group can be stored in $O(n^\epsilon)$ space. Therefore, we can perform any local computation on each group. Each group consists of several subtrees. We will show in Lemma~\ref{lem:lastsub} that for each group, all but one subtree can be efficiently compressed into a single bit ($d(v)$ for root $v$). The final subtree can be compressed (visually, on our tree, we are contracting this entire subtree) into an encoding equal to the number of unknown dependencies it has by Theorem~\ref{thm:compress}, which is at most $n^\epsilon$ by assumption. Since this step is all local, it requires 1 round.
    %\item Since all but one of the subtrees in a group can be entirely solved, we will take the opportunity at the end of the preprocessing to simplify using these subtrees. Each group sends its completed subtrees to the the parents of the subtree. For each parent, it will compute its value based off its children. Since the degree of a parent may be large, this could take $O(1/\epsilon)$ rounds. After that, we will repeat step 3 once with these new completed values to further compress the remaining components in groups. \hamed{Is it just once or multiple times? If so for how many times? and why repeating step 3 is necessary?}\marina{once. i found that repeating it is necessary to actually get rid of all but the last component in a group. otherwise groups can still have more than $n^{1-\epsilon}$ dependencies.} This step ensures that there remains only one compressed node per group after preprocessing.
    \item Finally, we run our compression algorithm to compress any vertex in the tree with a leaf. Then, we get that vertex in terms of all of its non-leaf children (which is at most $n^\epsilon$ by assumption), and we can remove all leaves.
\end{enumerate}


%In step 2, we consider every big node $v$ with at most $n^\epsilon$ children who depend on a big node. A child $u$ of $v$ depends on a big node if either $u$ itself is a big node or it has a descendent that is a big node. We will later show that the vast majority of big nodes will exhibit this property. For each such $u$, we will later show that its underlying subtree's number of dependencies has reduced by a factor of $n^\epsilon$ in the preprocessing step. This allows us to recurse on $u$'s subtree. \hamed{It's not clear to me how this recursion works. Do we run the entire algorithm (including or excluding preprocessing step?) on each child $u$ of a big node $v$ such that $u$ depends on another big node? Does this subtree include other big nodes too? And in that case, do we run another instance of the algorihtm on the children of those big nodes within $u$'s subtree?} \marina{i defined $u$ to be a child of a big node with no dependencies on big nodes. that means that the subtree rooted at $u$ has no big nodes in it}By induction, we will show this requires $O\left(((1-i\epsilon)/\epsilon)^{(1-i\epsilon)/\epsilon}\right)$ rounds during phase $i$. \hamed{Is there any proof or explanation for this?}\marina{that is one of the leftover proofs}

%Finally, in step 3, we will compress most of the big nodes. As stated before, we will show that most of the big nodes have at most $n^\epsilon$ children who depend on another big node, and all other children were compressed to a single bit, $d(v)$ for root $v$, in step 2. \hamed{Wait, in step $2$, do we recurse on vertices $u$ that depend on a big node or is it reverse ($u$ does not depend on a big node)?}\marina{does not depend on a big node} Therefore, our big node now has at most $n^\epsilon$ unknown children, and we already know that the size of these trees are at most $n^\epsilon$. Thus we can store them on their own machines and compress them so that they are now small in 1 round. This completes the phase.

%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.08]{tree-maximal-matching}
%    \caption{This figure shows the execution of one phase of the algorithm, assuming that the leaf-stars are not shrunk. The bold vertices are matched, and the red vertices are not isolated in the remaining graph.}
%\end{figure}

To finish the algorithm, after $1/\epsilon$ phases, we store the remaining graph on one machine and complete the computation of $d(v)$ for all $v$. Then by Lemma~\ref{lem:d(v)}, we can use these values to compute the maximum matching in $O(1/\epsilon)$ AMPC rounds in the specified space constraints. Now we must prove our assumptions to show that we end up with a maximum matching in the correct time and space. We do this assumption by assumption.
\fi

Ultimately, we prove Theorem~\ref{thm:dptwo} in order to achieve a versatile framework to automatically translate a vast range of tree-contraction-based algorithm into an $O(1/\epsilon)$ round AMPC counterpart.

\dptwo*

\begin{proof}
First, we present an algorithm for $\C^i$. We are given a connected subtree induced by $S = \{ v_1, v_2, \ldots, v_k \}$ of $T$ so that $\sum_{j=1}^k{w(v_j)} = O(i)$. Since $i = O(n^\epsilon)$, the whole subtree fits into the memory of a single machine. Some of the leaves of this subtree are \emph{known}, meaning that they are a leaf also in $T$, and others are \emph{unknown}, meaning that they have children outside $S$. Let $\mathcal{U} = \{ u_1, u_2, \ldots, u_l \}$ be the set of the children of \emph{unknown} leaves as well as the children of non-leaf nodes  which are outside of $S$. Ultimately, we want to compress the data already stored on the vertices of $S$ into a memory of $\widetilde{O}(l)$ as the degree of $v_1$ in the contracted tree $T'$ will be $l + 1$, and thus $w_{T'}(v_1) = l + 1$. 

The data we store on each contracted vertex $v_1$ is a tree structure $T^{\C}(v_1)$ whose leaves are the children of $v_1$ in $T'$, and there is no vertex with exactly one child in $T^{\C}(v_1)$. Thus, the number of vertices in $T^{\C}(v_1)$ is bounded by $O(l) = O(w_{T'}(v_1))$. In addition, we guarantee that there exists a data of size $\widetilde{O}(1)$ on each vertex of $T^{\C}(v_1)$ due to $\mathcal{G}^1$ being $w$-bounded for $w(v) = 1$. 
Therefore, we assume each vertex $v_j \in S$ is a contracted vertex which has stored a tree structure of size $\widetilde{O}(w_T(v_j))$ as its data. We concatenate all these trees to get an initial $T^{\C}(v_1)$ whose size is bounded by $\sum_{j=1}^k{\widetilde{O}(w_T(v_j))} = \widetilde{O}(n^\epsilon)$.

We run a $2$-tree-contraction-\emph{like} algorithm locally on $T^{\C}(v_1)$ using $\C^1$ and $\R^1$. Note that we can only rake the known leaves since the data of unknown leaves depend on their children. We repeating \compress{} and \rake{} stages until there is no known leaf or a vertex with one child remain in $T^{\C}(v_1)$. Then, according to Lemma~\ref{lemma:rounds} for $\alpha=2$, the number of remaining vertices in $T^{\C}(v_1)$ is bounded by $O(l)$. We store the final $T^{\C}(v_1)$ along with the data stored on each of its children as the data of $v_1$ in $T'$ which requires a memory of $\widetilde{O}(l) = \widetilde{O}(w_{T'}(v_1))$. Hence, $\C^i$ satisfies the $w$-bounded property for $w(v) = \degr(v)$.

Finally, we present an algorithm for $\R^i$ which is more straight-forward compared to that of $\C^i$. We are given a leaf-star $S = \{ v_1, v_2, \ldots, v_k \}$ of $T$ so that $\sum_{j=1}^k{w(v_j)} = O(i)$. This implies that there are at most $O(n^\epsilon)$ vertices in $S$ as long as $i = O(n^\epsilon)$, and we can fit the whole $S$ into a memory of a single machine. To simulate $\R^i$, we only need to $k-1$ times apply $\R^1$ on $S_j = \{ v_1, v_{j+1} \}$ at the $j$-th iteration. Note that every $v_j \in S$ is a  leaf in $T$, so the data stored for $v_j$ is just $\widetilde{O}(1)$ bits and not a tree structure. Theorem~\ref{thm:dptwo} statement is implied.
\end{proof}



==> utils-old.tex <==

\usepackage{amsfonts, amsmath, amssymb, amsthm, enumerate, gensymb, lastpage, mathtools, tikz, graphicx, thmtools, hyperref, url, thm-restate, cite}

\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\graphicspath{{images/}}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{xcolor}
\usepackage{pdftexcmds}
\usepackage{caption}
\usepackage{subcaption}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{observation}[lemma]{Observation}
\newcommand{\marina}[1]{\textcolor{red}{Marina: #1}}
\newcommand{\hamed}[1]{\textcolor{blue}{Hamed: #1}}
\newcommand{\hsinhao}[1]{\textcolor{green}{Hsin: #1}}

%\title{Constant Round Tree Contraction in AMPC}


\newcommand{\blackbox}[1]{\textsc{#1}}

%\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}

\usepackage{xcolor}


\newtheorem{defn}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{claim}{Claim}

%\setcounter{section}{-1}

%\newcommand{\lrp}[1]{\left( #1 \right)}
%\newcommand{\lrb}[1]{\left[ #1 \right]}
%\newcommand{\al}[1]{\begin{align*} #1 \end{align*}}
%\newcommand{\wt}[1]{\widetilde{ #1 }}
%\newcommand{\Bern}{\text{Bern}}
\newcommand{\noi}{\noindent}
%\newcommand{\marina}[1]{\textcolor{red}{Marina: #1}}
\newcommand{\data}{\mathcal{D}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\cycleconj}{\textsf{1-vs-2Cycle}}
\newcommand{\compress}{\blackbox{Compress}}
\newcommand{\rake}{\blackbox{Rake}}
\newcommand{\bigsmall}{$\alpha$-Big-Small tree}
\declaretheorem[name=Theorem]{thm}
\newcommand{\children}{\textsf{children}}
\newcommand{\leaves}{\textsf{leaves}}
\newcommand{\val}{\textsf{value}}
\newcommand{\sumparent}{\textsf{SumParent}}

